Joint Angular Refinement and Reconstruction for Single-Particle Cryo-EM

Single-particle cryo-electron microscopy (cryo-EM) reconstructs the three-dimensional (3D) structure of bio-molecules from a large set of 2D projection images with random and unknown orientations. A crucial step in the single-particle cryo-EM pipeline is 3D refinement, which resolves a high-resolution 3D structure from an initial approximate volume by refining the estimation of the orientation of each projection. In this work, we propose a new approach that refines the projection angles on the continuum. We formulate the optimization problem over the density map and the orientations jointly. The density map is updated using the efficient alternating-direction method of multipliers, while the orientations are updated through a semi-coordinate-wise gradient descent for which we provide an explicit derivation of the gradient. Our method eliminates the requirement for a fine discretization of the orientation space and does away with the classical but computationally expensive template-matching step. Numerical results demonstrate the feasibility and performance of our approach compared to several baselines.

==> CryoEM-Joint Reconstruction/sections/1-introduction.tex <==

Single-particle cryo-electron microscopy (cryo-EM) aims at obtaining the three-dimensional (3D) atomic structures of biological macromolecules such as proteins or viruses. Replicates of a molecule of interest, in unknown orientations, are first imaged at cryogenic temperatures. From those 2D projections (Figure~\ref{fig:intro_pic} left), one then reconstructs the 3D density map of the molecule (Figure~\ref{fig:intro_pic} right), a computational process named ``single-particle analysis'' (SPA). The reconstruction task in SPA is extremely challenging due to the lack of knowledge on the projection directions, heavy noise and the blurring inherent with the point spread function (PSF) of the microscope. To tackle this difficulty, most methods start by estimating an \textit{ab-initio} model from class-averaged particle images. Then, this initial model is refined iteratively until a high-resolution map is obtained, a task named ``3D refinement''. 

\begin{figure}[t!]
    \centering
    \begin{tikzpicture}
    \node at (0,0) {\hspace{-0.2cm}\includegraphics[width =  \linewidth]{figures/fig1_1.png}};
    \draw[white,fill=white] (-2.7,2.2) rectangle (4.5,2.6);
    \node at (-1.8,2.4) {\scriptsize (a) Ground truth};
    \node at (0,2.4) {\scriptsize (b) True orient.};
    \node at (1.6,2.4) {\scriptsize (c) Joint opt.};
    \node at (3.3,2.4) {\scriptsize (d) Unref. orient.};
    \end{tikzpicture}
    \caption{Single particle analysis. Left: Samples of the noisy projection images used in this experiment. Right: Comparison between the central slices of (a) the ground-truth, (b) the reconstruction from the true orientations, (c) the reconstruction obtained with our joint refinement method, (d) the reconstruction from the unrefined initial orientations.} 
    \label{fig:intro_pic}
\end{figure}


%------------------------------------
\subsection{Standard 3D Refinement Techniques}

Currently, state-of-the-art refinement techniques~\textcolor{black}{\cite{Scheres2012,punjani2017cryosparc,Xmipp2013,Grigorieff2007}} produce a high-resolution density map by alternating between
\begin{enumerate}
    \item the reconstruction of the 3D density map for a given set of (however inaccurate) projection orientations; 
    \item the refinement of the projection orientations for all 2D particles based on the previously reconstructed 3D volume. 
\end{enumerate}

The reconstruction problem can be solved using different approaches such as algebraic methods~\cite{Gordon1970, Gilbert1972}, weighted back-projection (WBP)~\cite{Radermacher2006}, direct Fourier methods~\cite{Penczek2004, Abrishami2015, Carazo2015}, and iterative regularized approaches~\cite{Nilchian2013, Jaitly2010, donati2018fast}. 

In most SPA packages, direct Fourier methods based on the central-slice theorem are used. Those methods work adequately when the projections are sufficiently numerous and their speed is a key advantage. Unfortunately, their use is less appropriate in the presence of heavy noise, few projection measurements, or inaccurately known projection angles. 

The past years have seen \textcolor{black}{the appearance} of more robust iterative schemes that formulate the 3D reconstruction problem as a regularized optimization problem and enable the incorporation of prior knowledge on the underlying signal~\cite{sorzano2017survey}. Their downside is that iterative schemes usually come with a prohibitive computational cost if not carefully engineered. 

Several works have considerably improved this situation by proposing methods with increased speed. In particular, an important breakthrough came when a costly step of many reconstruction algorithms was shown to be quickly computable as a discrete convolution~\cite{delaney1996fast,vonesch2011fast,donati2018fast}. 

For the angular-refinement task, the most commonly used method is projection-matching~\textcolor{black}{~\cite{penczek1994ribosome, Baker1996}}. It compares every projection image against a finite set of clean templates obtained from the current estimate of the 3D density map and then assigns the angular parameters based on the closest match~\cite{Heymann2007}. Projection-matching hence performs angular assignment on a discretized orientation space. As a consequence, the quality of the angular refinement depends on the fineness of the discretization and the quality of the density map used to generate the templates. One bottleneck is that a fine discretization comes at the cost of large set of templates, which leads to a computationally expensive procedure. Moreover, methods based on projection-matching were found to degrade significantly in low SNR regimes~\cite{Sigworth2015} or when errors occur in the estimation of the density map used for the generation of the clean templates \cite{Punjani2017}.

Examples of joint-reconstruction methods that address 3D \textit{ab initio} modeling are found in~\cite{Barnett2017}, \cite{yves2018}. In~\cite{Barnett2017}, a frequency-marching approach that increases the resolution of the reconstruction is proposed. This leads to a smaller computational overhead in projection-matching steps. In~\cite{yves2018}, the density map parameters are updated through gradient descent while the projection orientations are recovered through exhaustive search on an $SO(3)$ grid, followed by convex optimization. Although they provide efficient 3D \textit{ab initio} modeling, these methods still suffer from the shortcomings of projection-matching. 

Finally, a joint-reconstruction framework for 2D tomography with unknown projection orientations is proposed in~\cite{Cheik2017}. The problem is solved through simulated annealing, which strongly limits its applicability to 3D tomography due to its high computational cost.

%------------------------------------
\subsection{Maximum-Likelihood Methods}
\label{sec:ML methods}
Scheres followed a Bayesian approach in \cite{Scheres2012} to formulate the 3D refinement problem as a maximum marginalized \textit{a posterior} (MAP) estimation~\textcolor{black}{~\cite{scheres2012bayesian}} that is solved by expectation maximization~\cite{Dempster1977}. This method is less sensitive to the initial model and brings higher robustness in low SNR regimes. However, its high computational complexity limits its applicability. 

Punjani \textit{et al.} proposed a  computationally efficient framework in~\cite{Punjani2017}. They formulated the 3D refinement problem as a MAP estimation and solved it by stochastic average gradient descent. They also used importance sampling to further reduce the cost of computing the marginalized likelihood. 

An advantage of maximum-likelihood-based methods is that they do not limit a particle image to a unique angular class. This leads to increased robustness in high-noise regimes compared to projection-matching procedures. However, they still involve some form of discretization of the projection orientations. In particular, they necessitate an overly fine discretization of the 3D orientation space, as well as a compactly supported grid over $\mathbb{R}^2$ for in-plane translations. Moreover, the marginalization process is usually computationally expensive. 
%------------------------------------

\subsection{Contributions}

In this work, we present a angular-refinement method for single-particle cryo-EM that jointly recovers the 3D density map and the orientation of each projection. This joint optimization problem is solved by letting the alternating-direction method of multipliers (ADMM) and gradient-descent steps take turns to update the density map and the orientations, respectively. 

We use an explicit derivation of the gradient of the objective function (Theorem~\ref{th:grad}) to optimize the orientations over a continuous space. Hence, a key advantage of the proposed approach over usual methods is that it avoids one to resort to a fine discretization of $SO(3)$ for the orientations and $\mathbb{R}^2$ for the in-plane translations.  Moreover, the computationally expensive step of projection-matching is skipped. 

By using fast algorithms, we are able to efficiently refine 3D density maps from sets of projections with poor initial angular estimation. We illustrate in Figure~\ref{fig:intro_pic} the type of refinements obtained with our joint-optimization framework, compared to a few baselines.

The paper is organized as follows: We describe in Section~\ref{sec:imaging_model} the image-formation model. In Section~\ref{sec:methods}, we detail our joint-optimization framework. The experimental setup is described in Section~\ref{sec:exp_conditions} and results are presented in Section~\ref{sec:results}. Finally, we conclude this work in Section \ref{sec:conclusion}. 

%------------------------------------

\subsection{Notations}

Sequences from $\mathbb{Z}^d \rightarrow \mathbb{R}$ are denoted by $\mathrm{c}[\cdot]$. Then, sequence samples are $\mathrm{c}[\mathbf{k}]$ with $\mathbf{k}=(k_1,\dots,k_d)\in\mathbb{Z}^d$. Bold lowercase letters (\textit{e.g.}, $\mathbf{c}$) represent vectors while bold uppercase letters are reserved for matrices (\textit{e.g.}, $\mathbf{H}$). All vectors are assumed to be column vectors unless otherwise stated. The $\ell_1$ and $\ell_2$ norms of the vector $\mathbf{c}\in\mathbb{R}^N$ are defined as $\lVert \mathbf{c} \rVert_1 \coloneqq \sum_{n=1}^N\abs{\mathrm{c}_n}$ and $\lVert \mathbf{c} \rVert_2 \coloneqq \big(\sum_{n=1}^N\abs{\mathrm{c}_n}^2 \big)^\frac{1}{2}$, respectively. The spaces $\ell_2(\mathbb{Z}^d)$ and $L_2(\mathbb{R}^d)$ contain finite-energy sequences and functions, respectively. The proximal operator of a convex functional $\mathcal{R}: \mathbb{R}^N \rightarrow \mathbb{R}$ is defined as $\text{prox}_{\mathcal{R}}(\mathbf{z};\mu) \coloneqq \,\argmin_{\mathbf{s}}\left( \frac{1}{2} \lVert \mathbf{s}-\mathbf{z} \rVert_2^2 + \mu \mathcal{R}(\mathbf{s}) \right)$, with $\mu\in\mathbb{R}$. The Fourier transform of $f$ is $\widehat f$. \textcolor{black}{The reflection of a function $f$ is denoted $f^\vee = f(-\cdot)$.}
Finally, the projection orientations and the in-plane translations are referred to as ``latent variables''.  

==> CryoEM-Joint Reconstruction/sections/2-sys_model.tex <==
\label{sec:imaging_model}

%------------------------------------
\vspace{0.25cm}
\subsection{Imaging Model for a Single Orientation}

Let $V \in {L}_2(\mathbb{R}^3)$ denote the 3D density map of a molecule and let $\Omega_{\mathrm{2D}} \subset \mathbb{Z}^2$  be the discretized projection domain (see Figure~\ref{fig:angles}). The number of elements in $\Omega_\mathrm{2D}$ is $M = \sharp\Omega_\mathrm{2D}$.

We model a cryo-EM projection image $g: \Omega_\mathrm{2D} \rightarrow \mathbb{R}$ for an orientation $\bm{\uptheta} =(\theta_1,\theta_2,\theta_3) \in  [0,2\pi)\times [0,\pi]\times [0,2\pi) $ and an in-plane translation $\mathbf{t} = (t_\mathrm{1},t_\mathrm{2}) \in \mathbb{R}^2$ as
\begin{align}
g[\mathbf{m}]= (h * \mathcal{P}_{\bm{\uptheta}} (V) )(\bm{\Lambda}\mathbf{m}-\mathbf{t}) + \rm{\varepsilon}[\mathbf{m}],  \; 
\label{eq:image_form}
\end{align}
where $\bm{\Lambda} = \mathbf{diag}(\Delta_{\mathrm{1}},\Delta_{\mathrm{2}})$ is a diagonal matrix formed out of the sampling steps $\Delta_{\mathrm{1}}$ and $\Delta_{\mathrm{2}}$ of the projection domain and ${\varepsilon}: \Omega_\mathrm{2D} \rightarrow \mathbb{R}$ is an additive Gaussian white noise with zero mean and $\sigma^2$ variance. The operator $\mathcal{P}_{\bm{\uptheta}}:{L}_2(\mathbb{R}^3) \rightarrow {L}_2(\mathbb{R}^2)$ is the projection operator for the orientation $\bm{\uptheta}$ and $h \in {L}_2(\mathbb{R}^2)$ corresponds to the PSF of the microscope. The vectorization of $g$ is $\mathbf{g} = (g[\mathbf{m}])_{\mathbf{m} \in \Omega_{2D}}$ so that $\mathbf{g} \in \mathbb{R}^M$. The same goes for  $\varepsilon$  and $\bm{\varepsilon}$. 

\tdplotsetmaincoords{60}{110}
%
\pgfmathsetmacro{\rvec}{.8}
\pgfmathsetmacro{\thetavec}{30}
\pgfmathsetmacro{\phivec}{60}
%
\begin{figure}[t!]
\centering
\begin{tikzpicture}[scale=4,tdplot_main_coords]
    \coordinate (O) at (0,0,0);
    \draw[thick,->] (0,0,0) -- (1,0,0) node[anchor=north east]{$\mathbf{e}_1$};
    \draw[thick,->] (0,0,0) -- (0,1,0) node[anchor=north west]{$\mathbf{e}_2$};
    \draw[thick,->] (0,0,0) -- (0,0,1) node[anchor=south]{$\mathbf{e}_3$};
    \tdplotsetcoord{P}{\rvec}{\thetavec}{\phivec}
    \draw[-stealth,color=red] (O) -- (P);
    \draw[dashed, color=red] (O) -- (Pxy);
    \draw[dashed, color=red] (P) -- (Pxy);
    \tdplotdrawarc{(O)}{0.2}{0}{\phivec}{anchor=north}{$\theta_1$}
    \tdplotsetthetaplanecoords{\phivec}
    \tdplotdrawarc[tdplot_rotated_coords]{(0,0,0)}{0.5}{0}%
        {\thetavec}{anchor=south west}{$\theta_2$}
    \draw[dashed,tdplot_rotated_coords] (\rvec,0,0) arc (0:90:\rvec);
    \draw[dashed] (\rvec,0,0) arc (0:90:\rvec);
    \tdplotsetrotatedcoords{\phivec}{\thetavec}{0}
    \tdplotsetrotatedcoordsorigin{(P)}
    \draw[dashed,blue,tdplot_rotated_coords,-] (-.4,0,0)
        -- (.4,0,0) node[anchor=north west]{};
    \draw[dashed,blue,tdplot_rotated_coords,-] (0,-.4,0)
        -- (0,.4,0) node[anchor=west]{};
    \draw[blue,tdplot_rotated_coords,-]  (-.4,.4,0) -- (.4,.4,0)  -- (.4,-.4,0) -- (-.4,-.4,0) -- (-.4,.4,0)   node[anchor=north]{};
    \tdplotdrawarc[tdplot_rotated_coords]{(0,0,0)}{0.2}{0}%
        {30}{anchor=north west,color=black}{$\theta_3$}
    \tdplotsetrotatedcoords{\phivec}{\thetavec}{30}
    \draw[thick,tdplot_rotated_coords,->] (0,0,0)
        -- (.3,0,0) node[anchor=north west]{$\mathbf{v}_1$};
    \draw[thick,tdplot_rotated_coords,->] (0,0,0)
        -- (0,.3,0) node[anchor=west]{$\mathbf{v}_2$};
    \node[blue] at (0.4,0.45,1.2) {$\Omega_{\mathrm{2D}}$};    
    \tdplotsetrotatedthetaplanecoords{45}
\end{tikzpicture}
\caption{3D Geometry of the imaging model for an orientation~$\boldsymbol{\uptheta}=(\theta_1,\theta_2,\theta_3)$. The Euler angles $\theta_1$, $\theta_2$, and $\theta_3$ represent the rotation, the tilt, and the in-plane rotation in the projection plane, respectively.}
\label{fig:angles}
\end{figure}

%------------------------------------
\subsection{Discretization}

To discretize the 3D density map $V$, we follow a generalized sampling scheme~\cite{Unser2000} and define
% --- Equation
\begin{equation}
V(\mathbf{x}) = \sum\limits_{\mathbf{k} \in \mathbb{Z}^3} {c}[\mathbf{k}] \varphi({\mathbf{x}}-\mathbf{k}), \; \forall \mathbf{x} \in \mathbb{R}^3,\label{eq:sampling}
\end{equation}
% ---
where $\varphi \in {L}_2(\mathbb{R}^3)$ is a given basis function and $c[\cdot] \in \ell_2(\mathbb{Z}^3)$ is a sequence that contains the coefficients of $V$ in the reconstructing space. The sampling step in the object domain is assumed to be equal to one, without loss of generality.

In this work, we choose $\varphi$ to be the optimized Kaiser-Bessel window function (KBWF)~\cite{Nilchian2015}
    \begin{equation}\label{eq:KBWF}
       \mkern-12mu  \varphi(\mathbf{x}) \mkern-2mu  =  \mkern-2mu \left\lbrace \mkern-10mu
        \begin{array}{ll}
              \frac{\beta_a(\|\mathbf{x}\|)^m  I_m\left(\alpha \beta_a(\|\mathbf{x}\|) \right)}{I_m(\alpha)},   \mkern-10mu &  \|\mathbf{x}\| \in [0,a] \\
           0,  & \text{otherwise} ,
        \end{array} \right. 
    \end{equation}
where $\beta_a(r)= \sqrt{1 - \left({r}/{a}\right)^2} $, $a>0$ is the support radius, $\alpha>0$ the window taper, and $I_m$ the modified Bessel function of order $m$.
KBWFs are well suited for tomographic reconstruction in reason of their isotropy and compact support~\cite{Nilchian2015, donati2018fast}. Moreover, the x-ray transform of KBWF does not depend on the orientation $\bm{\uptheta}$ and admits a closed-form expression~\cite{Lewitt1990}. It was shown in~\cite{Nilchian2015} that a KBWF represents functions very effectively when using specific parameter values (\textit{e.g.},  $m=2$, $a=4$, and $\alpha=19$).
% As suggested in~\cite{Nilchian2015}, we use the optimized parameters of the KBWF which leads to smaller deviation from partition of unity is beneficial for the reconstruction.

Because the density map $V$ is compactly supported, the sequence  $c[\cdot] \in \ell_2(\mathbb{Z}^3)$ can be restricted to a finite number of nonzero coefficients $\mathbf{c}=({c}[\mathbf{k}])_{\mathbf{k}\in \Omega_{\mathrm{3D}}}$, where $\Omega_{\mathrm{3D}} \subset \mathbb{Z}^3$ and $N = \sharp\Omega_\mathrm{3D}$. 

We then substitute \eqref{eq:sampling} in \eqref{eq:image_form}, and use the linearity and the pseudo-translation invariance of the x-ray transform~\cite{Natterer2001} to obtain a discrete version of the forward model, as in
\begin{align}
\mkern-5mu {g}[\mathbf{m}] & = \mkern-12mu \sum\limits_{\mathbf{k} \in \Omega_{\mathrm{3D}}}  \mkern-9mu  {c}[\mathbf{k}] (h * \mathcal{P}_{\bm{\uptheta}} (\varphi) )(\bm{\Lambda}\mathbf{m} - \mathbf{M}_{\bm{\uptheta}^\perp} \mathbf{k} - \mathbf{t}) + \varepsilon[\mathbf{m}]. \label{eq:disc_forward}
\end{align}
Here, $\mathbf{M}_{\bm{\uptheta}^{\perp}} \in \mathbb{R}^{2 \times 3}$ is the orthogonal projector operator
\begin{equation}
\mathbf{M}_{\bm{\uptheta}^{\perp}} \mkern-5mu = \mkern-5mu   \begin{pmatrix} C_1C_2C_3 - S_1S_3 & \mkern-5mu C_3S_1+C_1C_2S_3 & \mkern-5mu-C_1S_2 \\ 
-C_1S_3-C_2C_3S_1 & \mkern-5muC_1C_3 - C_2S_1S_3 & \mkern-5mu S_1S_2 \end{pmatrix}, \label{eq:M_omega}
\end{equation}
where $\forall i = \{1,2, 3\}, \, C_i = \cos(\theta_i)$ and $S_i=\sin(\theta_i)$.

Finally, we write \eqref{eq:disc_forward} as
\begin{equation}
    \mathbf{g} = \mathbf{H}(\bm{\uptheta},\mathbf{t}) \, \mathbf{c}+ \mathrm{\bm{\upvarepsilon}}, \label{eq:linear_proj_model}
\end{equation}
where $\mathbf{H}(\bm{\uptheta},\mathbf{t}) \in \mathbb{R}^{M \times  N}$ is the discrete imaging operator for orientation $\bm{\uptheta}$ and in-plane translation $\mathbf{t}$.

%------------------------------------
\subsection{Global Imaging Model}

We now consider a set of $P$ projection images (indexed as $\mathbf{g}_p$) such that $\mathbf{g}=\{\mathbf{g}_p \in \mathbb{R}^{M} \}_{p =1}^P$. Similarly, the set of projection orientations is defined as $\boldsymbol{\Theta} = \{\bm{\uptheta}_p\in \Theta \}_{p =1}^P$ and the set of in-plane translations as $\boldsymbol{\Gamma}=\{\mathbf{t}_p\in \mathbb{R}^2 \}_{p =1}^P$. 

The global imaging model is thus given by
\begin{align}
\label{equ:global-imaging-model}
    \mathbf{g} = \mathbf{H}(\boldsymbol{\Theta}, \boldsymbol{\Gamma}) \, \mathbf{c}+ \bm{\upvarepsilon},
\end{align}
where \begin{equation}
   \mathbf{g} = \begin{bmatrix}
                \mathbf{g}_1 \\ \vdots \\ \mathbf{g}_P
                \end{bmatrix}, \; 
    \mathbf{H}(\boldsymbol{\Theta}, \boldsymbol{\Gamma}) =   
    \begin{bmatrix}
                \mathbf{H}(\bm{\uptheta}_1,\mathbf{t}_1) \\ \vdots \\ \mathbf{H}(\bm{\uptheta}_P,\mathbf{t}_P)
                \end{bmatrix}, 
    \bm{\upvarepsilon} = \begin{bmatrix}
                \bm{\upvarepsilon}_1 \\ \vdots \\ \bm{\upvarepsilon}_P
                \end{bmatrix}
\end{equation}

For the sake of clarity we shall thereafter use the notations  $\mathbf{H}^T\mathbf{H}(\boldsymbol{\Theta}, \boldsymbol{\Gamma})=(\mathbf{H}(\boldsymbol{\Theta}, \boldsymbol{\Gamma}))^T\mathbf{H}(\boldsymbol{\Theta}, \boldsymbol{\Gamma})$ and $\mathbf{H}^T(\boldsymbol{\Theta}, \boldsymbol{\Gamma}) = (\mathbf{H}(\boldsymbol{\Theta}, \boldsymbol{\Gamma}))^T$.

==> CryoEM-Joint Reconstruction/sections/3-methodology.tex <==
\label{sec:methods}

% ========================================================

\subsection{Joint-Optimization Framework}

Our goal is to jointly estimate the unknown variables in~\eqref{equ:global-imaging-model}, which are the coefficients~$\mathbf{c}$ of the density map, the projection orientations $\boldsymbol{\Theta}$, and the in-plane translations $\boldsymbol{\Gamma}$. To do so, we express the refinement procedure as a regularized least-squares minimization
% --- Equation 
\begin{equation}
   \big(\hat{\mathbf{c}}, \hat{\boldsymbol{\Theta}}, \hat{\boldsymbol{\Gamma}}\big) \in \left\lbrace \mathrm{arg} \, \underset{\mathbf{c},\boldsymbol{\Theta}, \boldsymbol{\Gamma}}{\mathrm{min}}  \;    \mathcal{J}\big(\mathbf{c}, \boldsymbol{\Theta}, \boldsymbol{\Gamma}\big) \right\rbrace, \label{eq:opt}
\end{equation}
% ---
where 
% --- Equation 
\begin{equation}
    \mathcal{J}\big(\mathbf{c}, \boldsymbol{\Theta}, \boldsymbol{\Gamma}\big) = \frac{1}{2} \Vert \mathbf{g} - \mathbf{H}(\boldsymbol{\Theta}, \boldsymbol{\Gamma}) \, \mathbf{c}\Vert_2^2+ \lambda \mathcal{R}( \mathbf{L} \mathbf{c}).
    \label{eq:funcOpt}
\end{equation}
% ---
Here, $\mathcal{R}$ is a sparsity-promoting functional and $\mathbf{L}$ a linear operator. Together, they are used to inject prior knowledge into the reconstruction process. As an example, setting $\mathbf{L}=\bm{\nabla}$ (i.e., the gradient operator) and $\mathcal{R}=\|\cdot\|_{2,1}$ leads to the popular total-variation (TV) regularization~\cite{rudin1992nonlinear}. The regularization parameter $\lambda$ controls the balance between the data-fidelity and the regularization terms. 

To solve \eqref{eq:opt}, we alternate between the minimization over $\mathbf{c}$ and the minimization over $\boldsymbol{\Theta}$ and $\boldsymbol{\Gamma}$. Although the objective function in \eqref{eq:opt} is convex with respect to $\mathbf{c}$, it is not convex with respect to the latent variables $\boldsymbol{\Theta}$ and $\boldsymbol{\Gamma}$. Moreover, it is smooth with respect to $\boldsymbol{\Theta}$ and $\boldsymbol{\Gamma}$, but usually not smooth (due to $\mathcal{R}$) with respect to $\mathbf{c}$. This dictates the choice of two different minimization procedures within the proposed alternating scheme. 

For the minimization of $\mathcal{J}$ with respect to $\mathbf{c}$, we use ADMM~\cite{Boyd2011}, which allows us to split the problem into a sequence of simpler subproblems (see Section~\ref{sec:update_c}). Then, taking benefit from the differentiability of $\mathcal{J}$ with respect to $\boldsymbol{\Theta}$ and $\boldsymbol{\Gamma}$, the latent variables are updated using gradient-descent with line-search (see Section~\ref{sec:update_latent}). The outline of this joint optimization procedure is given in Algorithm~\ref{alg:refinement} and is implemented within the framework of the GlobalBioIm library\footnote{\texttt{http://bigwww.epfl.ch/algorithms/globalbioim/}}~\cite{soubies2018pocket}.

Note that, at Line~\ref{line:ADMM} of  Algorithm~\ref{alg:refinement}, we use the notation $\mathrm{ADMM}\left(\mathcal{J}( \cdot,\boldsymbol{\Theta}^k, \boldsymbol{\Gamma}^k), \mathbf{c}^{k} \right)$  to refer to the minimization of $\mathcal{J}( \cdot,\boldsymbol{\Theta}^k, \boldsymbol{\Gamma}^k)$ using ADMM initialized with~$\mathbf{c}^{k}$. We do the same for the gradient-descent algorithm (see Line~\ref{line:GD}). 
 
\begin{algorithm}[t]
  \caption{Joint-Optimization Framework
}
  \label{alg:refinement}
  %\ Initialize angles ($\bm{\theta}^0$,$\bm{\phi}^0$), shifts $\mathbf{T}^0$, and coefficients $\mathbf{c}^0$.
  \textbf{Require:} $\mathbf{c}^0$,$\bm{\Theta}^0$,$\bm{\Gamma}^0$
  \begin{algorithmic}[1]
    \State $k=0$
    \While {not converged} %{$k<K_\mathrm{max}$}
    \LineComment{Update the density map:}
    \State 
    $\mathbf{c}^{k+1} = \mathrm{ADMM}\left(\mathcal{J}( \cdot,\boldsymbol{\Theta}^k, \boldsymbol{\Gamma}^k), \mathbf{c}^{k} \right)$ \label{line:ADMM}
     \LineComment{Update the latent variables:} 
      \State 
      $ (\bm{\Theta}^{k+1},\bm{\Gamma}^{k+1}) =  \mathrm{GD}\left(\mathcal{J}( \mathbf{c}^{k+1},\cdot,\cdot), \bm{\Theta}^k,\mathbf{\Gamma}^k \right)$ \label{line:GD}
        \State $ k \gets k+1$
        \EndWhile
  \end{algorithmic}
   \textbf{Return:} $ \mathbf{c}^{k},\bm{\Theta}^{k}, \mathbf{\Gamma}^{k}$
\end{algorithm}


% ========================================================

\subsection{Update of the Density Map} \label{sec:update_c}

Given $\boldsymbol{\Theta}$ and $\boldsymbol{\Gamma}$, the reconstruction task consists in solving 
% --- Equation 
\begin{equation}
    \label{funcOpt-min-wrt-c}
    \hat{\mathbf{c}}= \textrm{arg} \min_{\mathbf{c}} \; \mathcal{J}(\mathbf{c},\boldsymbol{\Theta}, \boldsymbol{\Gamma}).
\end{equation}
% --- 
To do so, we use the ADMM scheme proposed in~\cite{donati2018fast}. The core idea is to split~\eqref{funcOpt-min-wrt-c} by introducing an auxiliary variable $\mathbf{u}$ so that
% --- Equation
\begin{align}
\label{eq:admm-minization-constrained}
\begin{split}
\hat{\mathbf{c}}= \textrm{arg} \min_{\mathbf{c}} & \; \left(\frac{1}{2} \Vert \mathbf{g} - \mathbf{H}(\boldsymbol{\Theta}, \boldsymbol{\Gamma}) \, \mathbf{c}\Vert_2^2 +\lambda \mathcal{R}(\mathbf{u}) \right) \\
 s.t. & \quad \mathbf{u}=\mathbf{L}\mathbf{c}.
\end{split}
\end{align} 
% ---
Then, the ADMM algorithm alternates between three steps, as summarized in Algorithm~\ref{alg:volume_update}. 

When TV regularization is used, the proximal operator at Line~\ref{algo:prox-u} admits a closed-form expression that can be computed efficiently~\cite{combettes2008proximal}. Then, the linear step at Line~\ref{algo:standard-admm-linear-step} is solved iteratively using a conjugate-gradient algorithm together with a fast formulation of the $\mathbf{H}^T\mathbf{H}(\boldsymbol{\Theta}, \boldsymbol{\Gamma})$ term~\cite{donati2018fast}. Finally, Line~\ref{admmcg-update-u} corresponds to a simple update of the dual variable $\widetilde{\mathbf{u}}$, while $\rho>0$ is a penalty parameter.

For the sake of completeness, the full set of equations behind the reconstruction algorithm is provided in Appendix~\ref{subsec:appendix-ADMM}.

% --- ALGORITHM 
\begin{algorithm}[t]
\caption{ADMM (Update of the Density Map)}
\label{alg:volume_update}
\vspace{0.1cm}
\textbf{Require:} $\mathbf{g}$, $\boldsymbol{\Theta}$, $\boldsymbol{\Gamma}$, $\mathbf{c}^0$, $\rho>0$ 
\begin{algorithmic}[1]
\State $\mathbf{u}^0= \mathbf{Lc}^0$, $\tilde{\mathbf{u}}^0= \mathbf{u}^0$
\State $k=0$ 
\While {$k < K_{\tiny \mathrm{ADMM}}$}
\State $\mathbf{u}^{k+1} = \text{prox}_{\mathcal{R}}\big(\mathbf{L}\mathbf{c}^k-{\widetilde{\mathbf{u}}^k}/{\rho}; \, {\lambda}/{\rho}\big)$ \label{algo:prox-u} 
\State $\mathbf{b} = (\mathbf{H}(\boldsymbol{\Theta}, \boldsymbol{\Gamma}))^T \mathbf{g} + \rho \mathbf{L}^T (\mathbf{u}^{k+1} - \tilde{\mathbf{u}}^k/\rho)$
\State $\mathbf{c}^{k+1} = \left(\mathbf{H}^T\mathbf{H}(\boldsymbol{\Theta}, \boldsymbol{\Gamma}) + \rho \mathbf{L}^T \mathbf{L} \right)^{-1} \mathbf{b}$ \label{algo:standard-admm-linear-step}
\State $\widetilde{\mathbf{u}}^{k+1} = \widetilde{\mathbf{u}}^{k}+\rho\big(\mathbf{u}^{k+1}-\mathbf{L}\mathbf{c}^{k+1}\big)$ \label{admmcg-update-u} 
\State $k\gets k+1$ 
\EndWhile
\end{algorithmic}
\textbf{Return:} $\mathbf{c}^{ K_{\tiny \mathrm{ADMM}}}$
\end{algorithm}

% ========================================================

\subsection{Update of the Latent Variables} \label{sec:update_latent}

   Let us first remark that the least-squares term in~\eqref{eq:funcOpt} can be written as
   \begin{equation}
        \frac{1}{2} \Vert \mathbf{g} - \mathbf{H}(\boldsymbol{\Theta}, \boldsymbol{\Gamma}) \, \mathbf{c}\Vert_2^2 = \frac{1}{2} \sum_{p=1}^P \|\mathbf{g}_p - \mathbf{H}(\bm{\uptheta}_p,\mathbf{t}_p) \, \mathbf{c} \|_2^2.
   \end{equation}
   Hence, when $\mathbf{c}$ is fixed, the minimization of $\mathcal{J}(\mathbf{c},\cdot,\cdot)$ amounts to solve
   \begin{equation}
       (\hat{\bm{\uptheta}}_p, \hat{\mathbf{t}}_p)  \in \left\lbrace    \mathrm{arg} \min_{\bm{\uptheta}, \mathbf{t}} \;\mathcal{J}_p(\bm{\uptheta}, \mathbf{t}) \right\rbrace \label{eq:latentVarOpt}
   \end{equation}
    for all $ p \in \{1,\ldots,P\}$, where  $\mathcal{J}_p : (\bm{\uptheta}, \mathbf{t}) \mapsto \mathbb{R}$ is defined as
   \begin{equation}
        \mathcal{J}_p(\bm{\uptheta},\mathbf{t}) = \frac{1}{2} \Vert \mathbf{g}_p - \mathbf{H}(\bm{\uptheta}, \mathbf{t}) \, \mathbf{c}\Vert_2^2.
        \label{eq:latentVarOpt-objFunction}
   \end{equation}
   As the objective function $\mathcal{J}_p$ is differentiable, the minimization in~\eqref{eq:latentVarOpt} can be achieved using gradient-descent steps. 
   {\color{black}
   Hence, we first need to compute the gradients
   \begin{align}
       & \bm{\nabla}_{\bm{\uptheta}}  \mathcal{J}_p(\bm{\uptheta}, \mathbf{t}) =  \left( \frac{ \partial \mathcal{J}_p}{\partial \theta_1}(\bm{\uptheta}, \mathbf{t}) , \frac{ \partial \mathcal{J}_p}{\partial \theta_2}(\bm{\uptheta}, \mathbf{t}) , \frac{ \partial \mathcal{J}_p}{\partial \theta_3}(\bm{\uptheta}, \mathbf{t})  \right) \label{eq:PartialTheta} \\
       & \bm{\nabla}_{\mathbf{t}}\mathcal{J}_p(\bm{\uptheta},\mathbf{t}) = \left( \frac{ \partial \mathcal{J}_p}{\partial t_1}(\bm{\uptheta}, \mathbf{t}), \frac{ \partial \mathcal{J}_p}{\partial t_2}(\bm{\uptheta}, \mathbf{t}) \right). \label{eq:PartialT}
   \end{align}
   
%   For $u \in \{1,2,3\}$ and $v \in \{1,2\}$, we have
%     \begin{align}
%       & \frac{ \partial \mathcal{J}_p}{\partial \theta_u}(\bm{\uptheta}, \mathbf{t})  = \left(\mathbf{H}(\bm{\uptheta},\mathbf{t}) \, \mathbf{c} -\mathbf{g}_p \right)^T  \left(\bm{\nabla}_{\theta_u} \mathbf{H}(\bm{\uptheta},\mathbf{t})\right) \mathbf{c}, \label{eq:PartialTheta2} \\
%       & \frac{ \partial \mathcal{J}_p}{\partial t_v}(\bm{\uptheta}, \mathbf{t}) =   \left( \mathbf{H}(\bm{\uptheta},\mathbf{t}) \, \mathbf{c} - \mathbf{g}_p\right)^T  \left(\bm{\nabla}_{t_v} \mathbf{H}(\bm{\uptheta},\mathbf{t})\right) \mathbf{c}, \label{eq:PartialT2}
%     \end{align}
%   where $\bm{\nabla}_{\theta_u} \mathbf{H}(\bm{\uptheta},\mathbf{t}) \in \mathbb{R}^{M \times N}$ \big($\bm{\nabla}_{t_v} \mathbf{H}(\bm{\uptheta},\mathbf{t}) \in \mathbb{R}^{M \times N}$, respectively\big) corresponds to the element-wise derivative of the matrix $\mathbf{H}(\bm{\uptheta},\mathbf{t})$ with respect to $\theta_u$ \big($t_v$, respectively\big).
   

   The explicit expressions of these  quantities are provided in Theorem~\ref{th:grad}. 
   \begin{theorem}\label{th:grad} Let $\varphi$ be an isotropic kernel and $\mathbf{H}(\bm{\uptheta},\mathbf{t}) \in \mathbb{R}^{M \times N}$ be defined by~\eqref{eq:disc_forward}.  Then, for $v \in \{\theta_1,\theta_2,\theta_3,t_1,t_2\}$, there exists $\mathbf{r}_v \in \mathbb{R}^N$ and $\mathbf{q}_v \in \mathbb{R}^N$ such that
   \begin{equation}\label{eq:thGrad}
       \frac{ \partial \mathcal{J}_p}{\partial v}(\bm{\uptheta}, \mathbf{t}) = \frac12 \mathbf{c}^T \left( \mathbf{r}_v \ast \mathbf{c} - 2 \mathbf{q}_v \right).
   \end{equation}
    Moreover, $\forall \mathbf{k} \in \Omega_\mathrm{3D}$,\\
        $\bullet$ if $v = \theta_i$ for $i \in \{1,2,3\}$,
         \begin{align}
                &{r}_v[\mathbf{k}] =  \frac{1}{\mathrm{det}(\bm{\Lambda})} \left( \frac{\partial \mathbf{M}_{{\bm{\uptheta}}^{\perp}} }{\partial \theta_i}   \mathbf{k} \right)^{T} \mkern-10mu \bm{\nabla} \left( \psi \ast \psi^\vee \right) (\mathbf{M}_{\bm{\uptheta}^{\perp}} \mathbf{k}), \\
                 \mkern-8mu & {q}_v[\mathbf{k}] = \frac{1}{\mathrm{det}(\bm{\Lambda})}  \bigg( \frac{\partial \mathbf{M}_{{\bm{\uptheta}}^{\perp}} }{\partial \theta_i}   \mathbf{k} \bigg)^{\mkern-3mu T} \mkern-5mu  \bm{\nabla}(g_p \ast \psi^\vee)  (\mathbf{M}_{\bm{\uptheta}^{\perp}} \mathbf{k}+\mathbf{t}),
        \end{align}
        $\bullet$ if $v = t_j$ for $j \in \{1,2\}$,
        \begin{align}
             &{r}_v[\mathbf{k}] = 0, \\
            &{q}_v[\mathbf{k}] = \frac{1}{\mathrm{det}(\bm{\Lambda})}   \frac{\partial (g_p \ast \psi^\vee)}{\partial y_j} (\mathbf{M}_{\bm{\uptheta}^{\perp}} \mathbf{k} + \mathbf{t}) ,
        \end{align}
    where  $\psi : \mathbf{y}=(y_1,y_2) \mapsto (h * \mathcal{P}(\varphi))(\mathbf{y})$, $\frac{\partial  \mathbf{M}_{{\bm{\uptheta}}^{\perp}}}{\partial \theta_i} \in \mathbb{R}^{2 \times 3}$ contains the entry-wise derivatives of $\mathbf{M}_{{\bm{\uptheta}}^{\perp}}$, and $g_p$ denotes the continuous counterpart of $\mathbf{g}_p$ (\ie interpolated values). 
   \end{theorem}

The proof is given in Appendix~\ref{sec:ProofGrad} and includes details on the gradients of $\psi \ast \psi^\vee$ and $g_p \ast \psi^\vee$. In particular, we show that they depend on $\mathcal{P}(\varphi)$ and $ \frac{\partial \mathcal{P}(\varphi) }{\partial y_j}$ whose expressions are provided in Proposition~\ref{propo:KBWF} for the specific case of the KBWF $\varphi$ in~\eqref{eq:KBWF}.  
   }
   
    \begin{proposition} \label{propo:KBWF} For the KBWF $\varphi$ given in~\eqref{eq:KBWF}, we have
    \begin{align}
       & \mkern-8mu \mathcal{P}(\varphi)(\mathbf{y}) = aA \, \beta_a(\|\mathbf{y}\|)^{m+\frac12}  I_{m + \frac12} \mkern-5mu\left( \alpha \beta_a(\|\mathbf{y}\|) \right),  \\
        &  \mkern-8mu \frac{\partial \mathcal{P}(\varphi) }{\partial y_v}(\mathbf{y}) =  \mkern-5mu - \frac{\alpha y_vA }{a}\beta_a(\|\mathbf{y}\|)^{m-\frac12}  I_{m-\frac12}(\alpha \beta_a(\|\mathbf{y}\|)),
    \end{align}
    where $A=\frac{\sqrt{2\pi/\alpha}}{I_m(\alpha)}$.
    \end{proposition}
    
The proof is given in Appendix~\ref{sec:ProofKBWF}.  

Equipped with those gradient expressions, we deploy a semi-coordinate-wise gradient-descent to solve~\eqref{eq:latentVarOpt}, as summarized in Algorithm \ref{alg:angular_assignment}. At each iteration, the parameters $\bm{\uptheta}$ and $\mathbf{t}$ are updated sequentially, which allows for the use of different stepsizes between orientation and in-plane translation. This is crucial to account for the different dynamics between these two variables. Moreover, we use adaptive steps that are selected according to a backtracking line-search method~\cite{armijo1966,Nocedal2006}. Given  an initial value, the step is decreased through the parameter $\eta \in (0,1)$ until the cost that corresponds to the updated variable is smaller than its current value (conditions checked in Steps \ref{line:AlgoGD-1} and \ref{line:AlgoGD-2}).

Finally, to further accelerate the update of the latent variables, we divide the projection set $\{1,\ldots,P\}$ into mini-batches and process them in parallel. It is the separability of the objective function in~\eqref{eq:latentVarOpt}, related to the independence of projection images, that makes this parallelization possible.


\begin{algorithm}[t!]
  \caption{GD (Update of the Latent Variables)}
  \label{alg:angular_assignment}
 \textbf{Require:} $\alpha^0_{\bm{\uptheta}}>0$, $\alpha^0_{\mathbf{t}}>0$, $\eta$ $\in (0,1)$, $\bm{\Theta}^0$, $\bm{\Gamma}^0$, $\mathbf{c}$
  \begin{algorithmic}[1]
    \NoDoFor{$p=1,\ldots,P$} 
    \State $k = 0$
    \NoDoWhile{$k < K_{\mathrm{GD}}$}
    \LineComment[2\dimexpr\algorithmicindent]{Update $\bm{\uptheta}_p$}
     \State $\alpha_{\bm{\uptheta}} \gets \alpha^0_{\bm{\uptheta}}$
    \State $\bm{\uptheta}^{k+1}_p = \bm{\uptheta}^{k}_p - \alpha_{\bm{\uptheta}} \bm{\nabla}_{\bm{\uptheta}} \mathcal{J}_p(\bm{\uptheta}_p^k,\mathbf{t}_p^k)$
    \NoDoWhile{$\mathcal{J}_p(\bm{\uptheta}_p^{k+1},\mathbf{t}_p^k) > \mathcal{J}_p(\bm{\uptheta}_p^k,\mathbf{t}_p^k)$} \label{line:AlgoGD-1}
    \State $\alpha_{\bm{\uptheta}} \leftarrow \eta \alpha_{\bm{\uptheta}}$
    \State $\bm{\uptheta}^{k+1}_p = \bm{\uptheta}^{k}_p - \alpha_{\bm{\uptheta}} \bm{\nabla}_{\bm{\uptheta}} \mathcal{J}_p(\bm{\uptheta}_p^k,\mathbf{t}_p^k)$
    \EndWhile
    \LineComment[2\dimexpr\algorithmicindent]{Update $\mathbf{t}_p$}
     \State $\alpha_{\mathbf{t}} \gets \alpha^0_{\mathbf{t}}$
    \State $\mathbf{t}^{k+1}_p = \mathbf{t}^{k}_p - \alpha_{\mathbf{t}} \bm{\nabla}_{\mathbf{t}} \mathcal{J}_p(\bm{\uptheta}_p^{k+1},\mathbf{t}_p^k)$
    \NoDoWhile{$\mathcal{J}_p(\bm{\uptheta}_p^{k+1},\mathbf{t}_p^{k+1}) > \mathcal{J}_p(\bm{\uptheta}_p^{k+1},\mathbf{t}_p^k)$}  \label{line:AlgoGD-2}
    \State $\alpha_{\mathbf{t}} \leftarrow  \eta \alpha_{\mathbf{t}}$
    \State $\mathbf{t}^{k+1}_p = \mathbf{t}^{k}_p - \alpha_{\mathbf{t}} \bm{\nabla}_{\mathbf{t}} \mathcal{J}_p(\bm{\uptheta}_p^{k+1},\mathbf{t}_p^k)$
    \EndWhile
    \State $k \gets k+1$
    \EndWhile
    \EndFor
  \end{algorithmic}
   \textbf{Return:} ${\bm{\Theta}}^{K_{\mathrm{GD}}},{\bm{\Gamma}}^{K_{\mathrm{GD}}}$
\end{algorithm}

{\color{black}
\subsection{Computational Complexity}
\label{sec:ComplexityComparaison}
We compare the computational complexity of the proposed latent variable update to that of projection matching.
Let $n$ and $m$ be such that $N = n^3$ and $M = m^2$ (\ie, $\mathbf{c} \in \mathbb{R}^{n \times n \times n}$ and $\mathbf{g}_p \in \mathbb{R}^{m \times m}$).

\subsubsection{Projection Matching}
Each iteration of projection matching consists of two steps.
\begin{itemize}
    \item \textit{Generation of Clean Templates.} Given the current density map $\mathbf{c}$, evaluate the forward model $\mathbf{H}(\bm{\uptheta},\mathbf{0}_{\mathbb{R}^2}) \, \mathbf{c}$ for $N_{\theta_1}N_{\theta_2}$ different values of $\bm{\uptheta}=(\theta_1,\theta_2,0)$ obtained by sampling $[0,2\pi)$ with $N_{\theta_1}$ points and $[0,\pi]$ with $N_{\theta_2}$ points. Denoting by $C_H$ the cost of one evaluation of the forward model, the computational complexity of this step is $O(N_{\theta_1}N_{\theta_2} C_H)$.
    \item \textit{Matching Projection Images $\mathbf{g}_p$.} Each projection image $\mathbf{g}_p$ ($p\in \{1,\ldots,P\}$) is compared against $N_{\theta_1}N_{\theta_2}$ clean templates. This requires rotation and in-plane translation alignment whose complexity is $O(m^2 \log m)$ if done efficiently using polar Fourier transform~\cite{Yang2008}, spherical harmonics~\cite{Lee2007}, or steerable basis functions~\cite{Zhao2014}.
\end{itemize}
The overall complexity of template matching is thus given by $O( N_{\theta_1} N_{\theta_2}( P m^2 \log m +  C_H))$. The cost of $C_H$ depends on its implementation. An efficient way to compute it can, for example, rely on the Fourier-slice theorem and the use of non-uniform FFT. This strategy roughly requires one 3D-FFT of the volume $\mathbf{c}$, one interpolation step to extract the central slice perpendicular  to  the  projection  direction, and one inverse 2D-FFT of this slice. This gives $C_H= n^3 \log n + m^2 + m^2 \log m$. With such an implementation, the overall complexity would thus be $O( N_{\theta_1} N_{\theta_2}( P m^2 \log m +  n^3 \log n))$.

\subsubsection{Proposed Update Scheme}
According to~\eqref{eq:thGrad} in Theorem~\ref{th:grad}, the evaluation of the partial derivative  $\partial \mathcal{J}_p / \partial v$ can be done at the cost of a 3D convolution (only required when $v=\theta_i$), a component-wise subtraction, and a scalar product. This gives a complexity of $O(n^3 \log n)$. To this has to be added the cost of computing $\mathbf{r}_v$ and $\mathbf{q}_v$ in Theorem~\ref{th:grad}. First, let us remark that $\frac{\partial  \mathbf{M}_{{\bm{\uptheta}}^{\perp}}}{\partial \theta_i}$ is known in closed form from~\eqref{eq:M_omega}. Hence, the complexity of computing $\frac{\partial  \mathbf{M}_{{\bm{\uptheta}}^{\perp}}}{\partial \theta_i} \mathbf{k}$ for all $\mathbf{k} \in \Omega_{\mathrm{3D}}$, is $O(n^3)$. Then, we distinguish two situations:
\begin{itemize}
    \item \textit{Explicit Expressions of $\bm{\nabla} \left( \psi \ast \psi^\vee \right) $ and}\footnote{Note that $\frac{\partial (g_p \ast \psi^\vee)}{\partial y_j}$ is nothing else than the $j$th component of $\bm{\nabla}(g_p \ast \psi^\vee)$.} \textit{$\bm{\nabla}(g_p \ast \psi^\vee)$ are Known}. Given $\bm{\uptheta}$ and $\mathbf{t}$, the computation of $\mathbf{r}_v$ and $\mathbf{q}_v$ amounts to their sampling at points $\mathbf{M}_{\bm{\uptheta}^{\perp}} \mathbf{k}$ (or $\mathbf{M}_{\bm{\uptheta}^{\perp}} \mathbf{k}+\mathbf{t}$), for $\mathbf{k} \in \Omega_{\mathrm{3D}}$, followed by a scalar product with $\frac{\partial  \mathbf{M}_{{\bm{\uptheta}}^{\perp}}}{\partial \theta_i} \mathbf{k}$, resulting in an overall complexity of~$O(n^3)$.
    \item \textit{Explicit Expressions of  $\bm{\nabla} \left( \psi \ast \psi^\vee \right) $ and $\bm{\nabla}(g_p \ast \psi^\vee)$ are Not Known}. Due to their independence upon $\bm{\uptheta}$ and $\mathbf{t}$, the relevant quantities can thus be evaluated \textit{once} (optionally upsampled) on the grid $\Omega_\mathrm{2D}$ using~\eqref{eq:GradPsiConvPsiVee} together with Proposition~\ref{propo:KBWF} and discrete convolutions (complexity of $O(m^2 \log m)$). Having this precomputed quantity saved as a lookup table, the evaluation of $\bm{\nabla} \left( \psi \ast \psi^\vee \right) $ and $\bm{\nabla}(g_p \ast \psi^\vee)$ at points  $\mathbf{M}_{\bm{\uptheta}^{\perp}} \mathbf{k}$ (or $\mathbf{M}_{\bm{\uptheta}^{\perp}} \mathbf{k}+\mathbf{t}$) is done by interpolation. Hence, here again, the computational complexity is $O(n^3)$.
\end{itemize}
Considering that there are~$P$ projection images and that $K_\mathrm{GD}$ iterations of gradient descent are performed at each update of the latent variables (see Algorithm~\ref{alg:refinement}), we obtain an overall complexity of $O(P K_\mathrm{GD} n^3 \log n)$. 

Finally, given that $K_\mathrm{GD}$ is typically small (for example in our experiments $K_\mathrm{GD}=3$) and that it is recommended~\cite{Sigworth2015} to set $N_{\theta_1}N_{\theta_2}$ in the order of $n^2$ to maintain a precise estimation of projection angles, the proposed method offers an interesting improvement in runtime over projection matching.
}

%===================================================================
% Discussion on Complexity between us
%===================================================================
% {\color{red}
% \subsection{Computational Complexity}
% Here we derive the computational complexity of one iteration of latent variable update using our method and compare it against projection matching. Let  $\mathbf{c} \in \mathbb{R}^{n \times n \times n}$ and $\mathbf{g}_p \in \mathbb{R}^{m \times m}$. Hence, $N = n^3$ and $M = m^2$. 
% % Note that the complexity of $\mathbf{H}(\bm{\theta}, \bf{t}) \bf{c}$ is $O(MN)$. 
% At each iteration of projection matching, we have the following steps:
% \begin{enumerate}
% \item Generate clean templates for $N_{\theta}$ orientations in $SO(3)$ and $N_t$ in-plane translations in $\mathbb{R}^2$. This amounts to evaluate the forward model (\ie $\mathbf{H}(\bm{\uptheta},\mathbf{t}) \, \mathbf{c}$) for  $N_{\theta}N_t$ couples $(\bm{\uptheta},\mathbf{t})$. \mz{I did not mention the computational complexity for computing the templates because this really depends on the implementation and whether we use Fourier based methods or our approach to generate projection templates.}\es{Ok, I added a sentence to say that it corresponds to the evaluation of the forward model. For my next comment I set that the cost of the fwd model if $C_H$.}
% \item Each projection image $\mathbf{g}_p$ ($p\in \{1,\ldots,P\}$) is then compared against $N_{\theta} N_t$ clean templates. This requires rotation and in-plane translation alignment which takes $O(m^3)$ or $O(m^2 \log m)$ if done efficiently using polar Fourier transform~\cite{Yang2008}, spherical harmonics~\cite{Lee2007} or steerable basis functions~\cite{Zhao2014}. Therefore, the computational cost of projection matching is $O(P N_\theta N_t m^2 \log m)$. \mz{I am not sure about the in-plane translations and whether they should appear in the final computational complexity or not. I guess it should not be included!}\es{Indeed I think that there is redundancy between points 1) and 2). From my understanding, there are two possibilities:
% \begin{enumerate}
%     \item Clean templates are generated by sampling only $\theta_1$ and $\theta_2$ (\ie not the in-plane rotations $\theta_3$, I think this corresponds to sampling S0(3), by the way it may be more clear to say discretizing $[0,2\pi]$ with $N_{\theta_1}$ points and $[0,2\pi]$ with $N_{\theta_2}$ points) and they are all centered (\ie no sampling of the translations, $\mathbf{t}=\mathbf{0}$). In this case $\mathbf{H}(\bm{\uptheta},\mathbf{t}) \, \mathbf{c}$ has to be evaluated $N_{\theta_1} N_{\theta_2}$ times. Then in step 2 each $\mathbf{g}_p$ is registered to each template (requiring in-plane rotations and translations) leading to the complexity  $O( N_{\theta_1} N_{\theta_2}( P m^2 \log m +  C_H))$. \mz{Agreed! :)}
%     \item Clean templates are generated by sampling $\theta_i$, $i=\{1,2,3\}$ (\ie $\bm{\uptheta}$) and $\mathbf{t}$, that is $N_{\theta_1} N_{\theta_2} N_{\theta_3} N_{\mathbf{t}}$ templates. In this case, in step 2, no registration is performed, only the error between the image $\mathbf{g}_p$ and the templates is computes $O(m^2)$. In this end we have $O( N_{\theta_1} N_{\theta_2} N_{\theta_3} N_{\mathbf{t}} (P m^2 + C_H) )$. 
% \end{enumerate}
% Hence I think the best is the first one and in that case indeed the in-plane translations should not appear in the final complexity (see a). Note also that the comparison of (a) and (b) is another example where it is preferable to not discretize (and thus use registration). \mz{I definitely agree with your point, we should use case (a) and remove $N_t$ from the computational cost for projection matching.} 
% Concerning the issue of the implementation of template generation, i.e. fwd computation, the question is : is there a method at least as efficient as $P m^2 \log m$ ? If yes we can omit this term. 
% \mz{An efficient way of obtaining the projections, would be to take non-uniform FFT of the volume and then take the central slice perpendicular to the projection direction (based on Fourier slice theorem). This also requires some interpolation from 2D polar to 2D uniform grid. The cost of taking FFT of the volume is $O(n^3 \log n)$ and taking the generation of all templates into account leads to $O(N_{\theta1} N_{\theta}_2 n^3 \log n)$. Lets assume that we use linear interpolation, then this will cost $O(m^2)$ or $O( N_{\theta}_1 N_{\theta}_2 m^2)$ for all the templates. Considering the computational cost of these two, leads to $O(N_{\theta1} N_{\theta}_2 n^3 \log n)$. Based on [19], $N_{\theta}$ is in the order of $n^2$. Thus leading to a computational cost of  $O( n^5 \log n)$. If $P<<n^2$, then the cost of generating the projection images will be dominant. Otherwise, the matching step between the projections and the templates would be dominant.}}
%\end{enumerate}
% As mentioned in~\cite{Sigworth2015}, to maintain a precise estimation of projection angles, $N_{\theta}$ is in the order of $n^2$. On the other hand, the dimension of the projection images is in the same order of the density map, i.e. $m = O(n)$.  Thus, the computational complexity of projection matching is $O(P N_t n^4 \log n)$.

% To derive the computational complexity of our method, let's consider the computation of the derivative of the loss with respect to one of the latent variables, for instance $\theta_u$, $u \in \{1, 2, 3\}$. For this purpose we expand equation \eqref{eq:PartialTheta2} as in,
% \begin{align}
% \frac{ \partial \mathcal{J}_p}{\partial \theta_u}(\bm{\uptheta}, \mathbf{t}) &= \mathbf{c}^T \mathbf{H}^T(\bm{\uptheta},\mathbf{t}) \bm{\nabla}_{\theta_u} \mathbf{H}(\bm{\uptheta},\mathbf{t}) \mathbf{c} -  \left(\bm{\nabla}_{\theta_u}\mathbf{H}^T  \mathbf{g}_p\right)^T \mathbf{c}
% \label{eq:expanded_loss_derivative}
% \end{align}
% Similar to~\cite{donati2018fast}, applying $\mathbf{H}^T \bm{\nabla}_{\theta_u} \mathbf{H}$ to $\mathbf{c}$ is performed by a convolution, reducing the computations to fast Fourier transformations (FFT) and inverse FFT \es{Should we write the result ? In particular provide the kernel of this convolution ?}. As a result, the computational complexity for the first term is $O(n^3 \log n)$ similar to~\cite{donati2018fast}. In addition, computing the kernel required for applying $\mathbf{H}^T \bm{\nabla}_{\theta_u} \mathbf{H}$ as a convolution is $O(P W^2 n)$ where $W$ is the number of discretizations for the support of the basis. Thus, computing the first term for all the projection images takes $O(P n^3 \log n + P W^2 n) = O(P n^3 \log n)$. 

% Following Theorem 2 in~\cite{donati2018fast}, $\bm{\nabla}_{\theta_u}\mathbf{H}^T  \mathbf{g}_p$ is done via 2D discrete convolution. Therefore, computing the second term for all the projection images in~\eqref{eq:expanded_loss_derivative} requires $O(P m^2 \log m + P n ^3) = O(P n^3)$ \es{I do not get the $Pn^3$}. Adding up the complexities corresponding to the first and second term leads to a computational complexity of $O(P n^3 \log n)$ for our approach. Compared to projection matching, our method is at least $N_t n$ times more efficient which is a significant gain for large sized density maps.  Note that the ultimate speed-up of our latent variables update compared to projection matching depends on the implementation details. However, comparing the computational complexity of updating the latent variables on a continuum and projection matching, further motivates the efficiency of our method. \mz{@Manu: Thanks a lot for the comments. I will add some notes to the draft which goes through the computational cost of various terms in more detail and also write downs the kernel for the new operators.}
% }

%\subsection{Computational cost of our method in more detail}
%  For now, let us only consider one of the terms involved in the update of the latent variables, i.e. $\frac{ \partial \mathcal{J}_p}{\partial \theta_u}(\bm{\uptheta}, \mathbf{t})$. Based on the definition in~\eqref{eq:latentVarOpt-objFunction}, $ \mathcal{J}_p(\bm{\uptheta}, \mathbf{t})$ is expanded as,
%  \begin{align}
% \mathcal{J}_p(\bm{\uptheta}, \mathbf{t}) = \frac{1}{2} \Vert \mathbf{g}_p \Vert^2 - \mathbf{g}_p^T \mathbf{H}(\bm{\uptheta}, \mathbf{t})\mathbf{c} + \frac{1}{2} \mathbf{c}^T \mathbf{H}^T(\bm{\uptheta}, \mathbf{t}) \mathbf{H}(\bm{\uptheta}, \mathbf{t}) \mathbf{c}.
%  \end{align}
%  Now taking the derivative of the above term with respect to $\theta_u$ leads to,
% \begin{align}
% \frac{ \partial \mathcal{J}_p}{\partial \theta_u}(\bm{\uptheta}, \mathbf{t}) = \frac{1}{2} \frac{\partial \left( \mathbf{c}^T \mathbf{H}^T(\bm{\uptheta}, \mathbf{t}) \mathbf{H}(\bm{\uptheta}, \mathbf{t}) \mathbf{c} \right)}{\partial \theta_u} - \frac{\partial \left( \mathbf{g}^T_p \mathbf{H}(\bm{\uptheta}, \mathbf{t}) \mathbf{c} \right)}{\partial \theta_u}.
% \label{eq:latentVarDeriv-expanded}
% \end{align}
% To derive the computational cost of our method, we look at the computational cost and the kernels involved in each individual term in~\eqref{eq:latentVarDeriv-expanded} .
% \vspace{5pt}

% \noindent \textbf{First term} $\frac{\partial \left( \mathbf{c}^T \mathbf{H}^T(\bm{\uptheta}, \mathbf{t}) \mathbf{H}(\bm{\uptheta}, \mathbf{t}) \mathbf{c} \right)}{\partial \theta_u}$: Based on equation A.4 in~\cite{donati2018fast},
% \begin{align}
% &\left[ \mathbf{H}^T(\bm{\uptheta}, \mathbf{t}) \mathbf{H}(\bm{\uptheta}, \mathbf{t}) \mathbf{c} \right]_\mathbf{k} = \nonumber \\ 
% &\sum\limits_{\bm{\ell} \in \mathbb{Z}^3} \mathbf{c}[\bm{\ell}] \left( \mathcal{P}(\varphi) * \mathcal{P}(\varphi) * h_p * h_p\right)(\mathbf{M}_{\mathbf{\theta}}^\perp (\bm{\ell} - \mathbf{k}))
% \end{align}
% where $h_p$ denotes the CTF of the microscope corresponding to projection image $p$. As a result, we have:
% \begin{align}
% & \mathbf{c}^T \mathbf{H}^T(\bm{\uptheta}, \mathbf{t}) \mathbf{H}(\bm{\uptheta}, \mathbf{t}) \mathbf{c} = \nonumber \\
% & \sum\limits_{\bm{\ell}, \mathbf{k} \in \mathbb{Z}^3} \mathbf{c}[\bm{\ell}] \mathbf{c}[\mathbf{k}] \left( \mathcal{P}(\varphi) * \mathcal{P}(\varphi) * h_p * h_p\right)(\mathbf{M}_{\mathbf{\theta}}^\perp (\bm{\ell} - \mathbf{k}))
% \end{align}
% Now we take derivative of the above term with respect to $\theta_u$,
% \begin{align}
% & \frac{\partial \left( \mathbf{c}^T \mathbf{H}^T(\bm{\uptheta}, \mathbf{t}) \mathbf{H}(\bm{\uptheta}, \mathbf{t}) \mathbf{c} \right)}{\partial \theta_u} \label{eq:deriv_ctHtHc} \\
% & = \sum\limits_{\bm{\ell}, \bm{k} \in \mathbb{Z}^3} \mathbf{c}[\bm{\ell}] \mathbf{c}[\mathbf{k}] \frac{\partial \left( \mathcal{P}(\varphi) * \mathcal{P}(\varphi) * h_p * h_p\right)(\mathbf{M}_{\mathbf{\theta}}^\perp (\bm{\ell} - \mathbf{k}))}{\partial \theta_u} \nonumber
% \end{align}
% where
% \begin{align}
% & \mathbf{r}_p[\mathbf{k}] = \frac{\partial \left( \mathcal{P}(\varphi) * \mathcal{P}(\varphi) * h_p * h_p\right)(\mathbf{M}_{\mathbf{\theta}}^\perp \mathbf{k})}{\partial \theta_u} \nonumber \\
% & = \left( \frac{\partial \mathbf{M}_{\theta^{\perp}}}{\partial \theta_u} \mathbf{k} \right)^T \nabla \left( \mathcal{P}(\varphi) * \mathcal{P}(\varphi) * h_p * h_p \right) (\mathbf{M}_{\theta^\perp}\mathbf{k}) \nonumber \\
% & = \left( \frac{\partial \mathbf{M}_{\theta^{\perp}}}{\partial \theta_u} \mathbf{k} \right)^T \left( \mathcal{P}(\varphi) * \nabla \mathcal{P}(\varphi) * h_p * h_p \right) (\mathbf{M}_{\theta^\perp}\mathbf{k}). \label{eq:kernel_rp}
% \end{align}
% As a result,~\eqref{eq:deriv_ctHtHc} is written as,
% \begin{align}
% \frac{\partial \left( \mathbf{c}^T \mathbf{H}^T(\bm{\uptheta}, \mathbf{t}) \mathbf{H}(\bm{\uptheta}, \mathbf{t}) \mathbf{c} \right)}{\partial \theta_u} = \mathbf{c}^T (\mathbf{r}_p * \mathbf{c}).
% \end{align}
% % Thus, once the kernel $\mathbf{r}_p$ is computed in~\eqref{eq:kernel_rp}, deriving $\mathbf{c}^T \left( \mathbf{r}_p * \mathbf{c}\right)$ takes $O(n^3 \log n)$ for computing the convolution and $O(n^3)$ for the computation of the inner product. Considering all the projection images leads to a computational cost of $O(P n^3 \log n)$. 
% On the other hand, the computational cost of computing the kernel involves computing $\mathcal{P}(\varphi) * \mathcal{P}(\varphi) * h_p * h_p$. If the basis function $\varphi$ is discretized on a grid of size $W \times W \times W$, then computing this kernel considering all the projection images takes $O(G W^2 \log W)$ where G corresponds to the number of CTF groups corresponding to the projection images and where $G<<P$ \mz{is this correct to have this assumption? Here I am assuming that all the projection images are coming from a few micrographs}.

% Thus, the total cost of deriving the first term is $O(P n^3 \log n + G W^2 \log W) = O(P n^3 \log n)$.

% \noindent \textbf{Second term} $\frac{\partial \mathbf{g}_p^T \mathbf{H}(\bm{\uptheta}, \mathbf{t})\mathbf{c}}{\partial \theta_u}$: The second term involves the following computations,
% \begin{align}
% \frac{\partial \mathbf{g}_p^T \mathbf{H}(\bm{\uptheta}, \mathbf{t})\mathbf{c}}{\partial \theta_u} = \frac{\partial \mathbf{c}^T  \mathbf{H}^T(\bm{\uptheta}, \mathbf{t}) \mathbf{g}_p}{\partial \theta_u}. 
% \end{align}
% Based on equation A.10 in~\cite{donati2018fast}, $\mathbf{H}^T(\bm{\uptheta}, \mathbf{t}) \mathbf{g}_p$ is written as,
% \begin{align}
% [\mathbf{H}^T(\bm{\uptheta}, \mathbf{t}) \mathbf{g}_p]_\mathbf{k} = \left( \mathbf{g}_p * \mathcal{P}(\varphi) * h_p \right)(\mathbf{M}_{\theta^\perp} \mathbf{k}). \label{eq:Htg_conv_form}
% \end{align}
% Now, by taking the derivative of~\eqref{eq:Htg_conv_form} with respect to $\theta_u$, we have
% \begin{align}
% \frac{\partial \mathbf{g}_p^T \mathbf{H}^T(\bm{\uptheta}, \mathbf{t})\mathbf{c}}{\partial \theta_u} &= \frac{\partial \sum\limits_{\mathbf{k}} \mathbf{c}[\mathbf{k}] (\mathbf{g}_p * \mathcal{P}(\varphi) * h_p)(\mathbf{M}_{\theta^\perp} \mathbf{k})}{\partial \theta_u} \\
% & = \sum\limits_{\mathbf{k}} \mathbf{c}[\mathbf{k}] \frac{\partial (\mathbf{g}_p * \mathcal{P}(\varphi) * h_p)(\mathbf{M}_{\theta^{\perp}} \mathbf{k}) }{\partial \theta_u}
% \end{align}
% Similar to the steps we took to determine the computational complexity of the first term, we have
% \begin{align}
% &\frac{\partial (\mathbf{g}_p * \mathcal{P}(\varphi) * h_p)(\mathbf{M}_{\theta^{\perp}} \mathbf{k}) }{\partial \theta_u} \\
% & = \left( \frac{\partial \mathbf{M}_{\theta^\perp}}{\partial \theta_u} \mathbf{k} \right)^T \mathbf{\nabla} \left( \mathbf{g}_p * \mathcal{P}(\varphi) * h_p \right) (\mathbf{M}_{\theta^\perp}\mathbf{k}) \nonumber \\
% & = \left( \frac{\partial \mathbf{M}_{\theta^\perp}}{\partial \theta_u} \mathbf{k} \right)^T \left( \mathbf{g}_p * \mathbf{\nabla} \mathcal{P}(\varphi) * h_p \right) (\mathbf{M}_{\uptheta^{\perp}}\mathbf{k})
% \end{align}
% The above expression is in the form of a 2D convolution which takes $O(P m^2 \log m)$, considering all the projection images. Also, taking into account the inner product between $\mathbf{c}$ and $\mathbf{H}(\uptheta, \mathbf{t})$, takes $O(P n^3)$. Therefore, the computational cost corresponding to the second term is $O(P m^2 \log m + P n^3) = O(P n^3)$.

% Aggregating the complexities of the first and the second terms results in $O(P n^3 \log n)$ as the computational cost of our method. Compared to projection matching, our method is $n$-times more efficient, which is a significant gain especially for large-sized density maps.
%=======================================================================================



==> CryoEM-Joint Reconstruction/sections/4-exp_conditions.tex <==
\label{sec:exp_conditions}

% ========================================================
\subsection{Datasets}

We test our algorithm on two synthetic datasets. The first dataset corresponds to the Holliday junction complex (HJC) density map, while the second corresponds to the Human patched 1 (PTCH1) protein. For each dataset, we generate the synthetic ground truth $V$ from the submitted density map~\cite{Laxmikanthan2016,Qi2018}, along with the associated atomic model in the Protein Data Bank using Chimera~\cite{Chimera2004}. The sizes of the HJC and PTCH1 volumes used in our simulations are $(90\times 90 \times 90)$ and $(84 \times 84 \times 84)$, \textcolor{black}{with voxel sizes of $2.867 \AA$ and $1.8 \AA$}, respectively. \textcolor{black}{We also synthesize a higher resolution version of  HJC with size $124\times124\times124$ and voxel size $2 \AA$. The first two volumes are used in our proof of concept simulations; the last volume is used in an experiment that mimics more realistic cryo-EM conditions (section V.E).} 

From those ground truths, we then generate $P$ projection images according to the image-formation model provided in~\eqref{eq:image_form}. We sample the orientation space using $P$ points in an equi-distributed fashion over $\{(\theta_{1,p},\theta_{2,p})\}_{p=1}^P$. The in-plane rotations are generated by uniformly sampling $P$ points on a $[0, 2\pi)$ interval. To perform in-plane translations, we move the center of the projection images randomly by at most $m_\mathbf{t}$ pixels in either horizontal or vertical directions. In our experiments, we use at most \textcolor{black}{$20000$}  projection images to demonstrate the feasibility of our method. Finally, the projection images are corrupted with additive Gaussian noise with zero mean and variance $\sigma^2$. The average signal-to-noise ratio (SNR) across all projection images is then given by $\mathrm{SNR}_{\mathrm{data}} = \frac{1}{P} \sum_{p=1}^P \frac{\Vert \mathbf{g}_p^\star\Vert_2^2}{\sigma^2}$ where $\mathbf{g}_p^\star$ correspond to noiseless measurements.

% ========================================================
\subsection{Initial Density Map, Orientations, and In-Plane Translations }

To generate an approximate density map from which to start the refinement procedure, we use the initial density map generated by 3D \textit{ab-initio} model in Relion~\cite{Relion2017}. For the projection orientations, we consider two possible initializations.
\begin{itemize}
    \item Model \textit{Init-1}: We add a zero-mean  random variable uniformly distributed in $[-e_{\theta},e_{\theta}]$ to the ground-truth orientations, \textit{i.e.}, ${\bm{\uptheta}}^{\mathrm{init}}_p = \bm{\uptheta}_p^{\mathrm{true}} + \bm{\upvarepsilon}_{\theta,p}$ where $\bm{\upvarepsilon}_{\theta,p,j} \sim \mathrm{Unif}(-e_{\theta},e_{\theta})$, $p \in \{1,\ldots,P\}$ and $j \in \{1,2,3\}$. 
    \item Model \textit{Init-2}: We use projection-matching (or another angular assignment method) to assign the initial projection orientations $\bm{\uptheta}^{\mathrm{init}}_p$, $p \in \{1,\ldots,P \}$. \textcolor{black}{For this initialization, we use the angular assignments from the 3D ab-initio modeling in Relion.}
\end{itemize}

The in-plane translations $\{\mathbf{t}_p\}_{p=1}^P$ are all initialized by zeros. With our notations we have that $\bm{\Theta}^\mathrm{init} = \{\bm{\uptheta}_p^\mathrm{init} \}_{p=1}^P$, $\bm{\Theta}^\mathrm{true} = \{\bm{\uptheta}_p^\mathrm{true} \}_{p=1}^P$, $\bm{\Gamma}^\mathrm{init} = \{\mathbf{0} \}_{p=1}^P$, and  $\bm{\Gamma}^\mathrm{true} = \{\mathbf{t}_p^\mathrm{true} \}_{p=1}^P$.

% ========================================================
\subsection{Tuning of the Hyper Parameters }
The parameters that need tuning are  $\lambda$, $\rho$, and $K_\mathrm{ADMM}$, as used in the update of the density map (Algorithm \ref{alg:volume_update}), and $\alpha_{\bm{\theta}}$, $\alpha_{\bm{t}}$, and $K_\mathrm{GD}$, as introduced in the update of the latent variables (Algorithm \ref{alg:angular_assignment}). In our experiments, we use $K_\mathrm{ADMM} = 2$ or $K_\mathrm{ADMM} = 5$, along with $K_\mathrm{GD} = 3$, $\alpha_{\bm{\uptheta}} = 10^{-7}$, $\alpha_{\bm{t}} = 10^{-5}$, and $\eta = 0.25$. The parameters $\lambda$ and $\rho$ grow like $\sigma$. We use the same set of parameters for the two molecules. Similar to \cite{donati2018fast}, the parameters of the KBWF used in the expansion of the volume in \eqref{eq:sampling}-\eqref{eq:KBWF} are $a=4$, $\alpha=19$, and $m=2$.

% ========================================================
\subsection{Metrics}

To assess the quality of reconstruction, we use the Fourier shell correlation (FSC) between the reconstructed volume $
V^\mathrm{rec}$ and the ground-truth $V^\mathrm{gt}$, as defined by
\begin{align}
\mathrm{FSC}(r) = \frac{\sum\limits_{r_i \in \textbf{r}} \hat{V}^\mathrm{rec}(r_i) \hat{V}^\mathrm{gt}(r_i)^*}{\sqrt{\sum\limits_{r_i \in \textbf{r}} \vert \hat{V}^\mathrm{rec}(r_i) \vert^2 \sum\limits_{r_i \in \textbf{r}} \vert \hat{V}^\mathrm{gt}(r_i) \vert^2} }.
\end{align}
where $\textbf{r} = \{(x_i, y_i, z_i): |\sqrt{x_i^2+y_i^2+z_i^2} - r |\leq \varepsilon_r\}$, for $\varepsilon_r >0$, denotes the set of all points in the discrete Fourier domain that lie in a  spherical shell with inner radius $r-\varepsilon_r$ and outer radius $r+\varepsilon_r$, centered at origin. The FSC thus computes the correlation between two corresponding spherical shells of the density maps in the Fourier domain. Moreover, we use the SNR metric defined as $\mathrm{SNR}(V^\mathrm{gt},V^\mathrm{rec})=20 \log_{10} \frac{\Vert V^\mathrm{gt} \Vert_2}{\Vert V^\mathrm{gt}-V^\mathrm{rec} \Vert_2}$.

To assess the quality of the 3D orientation refinements, we visualize the deviations of the refined angles from their ground-truth values. In other words, we examine the distribution of $\{\theta_{i,p}^{\mathrm{true}}-\theta_{i,p}^{\mathrm{rec}}\}_{p=1}^P$ for $i \in \{1,2,3\}$ and compare it to $\{\theta_{i,p}^{\mathrm{true}}-\theta_{i,p}^{\mathrm{init}}\}_{p=1}^P$. When the difference between the angles is small (up to some global rotations), the distribution of the differences is more concentrated around zero. On the contrary, the distribution is more expanded for angles that are further away from their ground-truth values.


\begin{figure*}[t]%\centering
\begin{minipage}{1\textwidth}
        % \includegraphics[width=1 \linewidth]{results/fullmodel_7795_masked_unif.png}
        \includegraphics[width=1 \linewidth]{results/7795_relion_wpost.png}
        \subcaption[first caption.]{PTCH1, $P=500$, $f_c = 0.03$, $\mathrm{SNR}_\mathrm{data} = 3.5781 \,(\textrm{dB})$, $m_{\bf{t}}=0$.}
        % \label{fig:fullmodel_7795}
\end{minipage}
\vfill%\hfil
\vspace{0.5cm}
    \begin{minipage}{1\textwidth}
    % \includegraphics[width=\hsize]{results/fullmodel_3400_masked_initrelion_unif.png}
    \includegraphics[width=\hsize]{results/3400_postprocessed.png}
    \subcaption[first caption.]{HJC, $P=500$, $f_c = 0.02$,  $\mathrm{SNR}_\mathrm{data} = -0.5733 \,(\textrm{dB})$, $m_{\bf{t}} = 3$.}
    % \label{fig:fullmodel-3400-1}
\end{minipage}
\vfill%\hfil
    \caption{Reconstructions of PTCH1 and HJC. {Left}: Samples of the noisy projection images.  Top row: 3D structures. Bottom row: Intensity maps of the central slice of the structures. The presented volumes are (a) the ground truth, (b) the initial map, (c) the reconstruction with unrefined projection orientations, (d) the output of our joint refinement approach, (e) the reconstruction with the true projection orientations, (f) the output of Relion \textcolor{black}{after post-processing}. For both experiments, the latent variables are initialized following the \textit{Init-1} model with $e_{{\theta}} = 0.7$ [rad].}
    \label{fig:fullmodel}
\end{figure*}


% ========================================================
\subsection{Compared Methods}

We compare our joint-optimization method to the following approaches:
\begin{enumerate}
\item \textit{Reconstruction with Unrefined Orientations}. We do not refine the initial angles and directly reconstruct the density map. This gives us an indication of the quality of reconstruction prior to the refinement procedure.  
\item \textit{Reconstruction with True Orientations}. We reconstruct the density map with the ground-truth orientations and in-plane translations. This serves as an oracle benchmark that allows us to quantify the improvement brought by our refinement procedure. 
\item \textit{Reconstruction with the Relion package}~\cite{Scheres2012}.
We run the \textit{3D auto-refine} function in Relion (version 2.1.0). The default parameters of this function (\textit{e.g.}, \textit{Initial angular sampling} and \textit{Local searches from auto sampling}) are used. For the particular experiments in which the in-plane translations are zero, the \textit{Initial offset range} and \textit{Initial offset step} parameters are set to their minimum values, which are $0$ and $0.1$, respectively. Otherwise, they are set to $4$ and $0.5$, respectively. Note that, to reduce the impact of noise when using Relion, we mask the projection images with a soft circular mask of a diameter that is proportional to the support of the density map.
\end{enumerate}

\textcolor{black}{All reconstructions from Relion are post-processed. We first apply a tight soft mask that embeds the maps. We then low-pass filter the volumes with a cut-off frequency that corresponds to the gold-standard FSC between the two half-maps; this is done using the post-processing function in Relion.}

% We also include a comparison with post-processed reconstructions obtained by filtering the noise outside a tight mask which encompasses the maps. The mask is obtained by applying a Gaussian filter to the refined map in Relion. The same mask is applied to the results of our joint-optimization method, reconstruction with true orientations and reconstruction with Relion.

 

==> CryoEM-Joint Reconstruction/sections/5-experiments.tex <==
\label{sec:results}


\section{Results}


%FSC----------------------------------------------------
% \begin{figure*}
% \centering
% 	\begin{tikzpicture}
% 		\begin{groupplot}[group style={group size= 2 by 3,                      % taille du group plot
%     					  horizontal sep=0.8cm, vertical sep=2cm},     
% 	            	 legend pos= north east,        % Position de la légende dans les figures
% 					 legend style={at={(0.995,0.99)},legend cell align=left},
% 					 grid=both,                         % grid
%     				 height=4cm,width=9cm,
%     				 xmin=0,xmax=0.5,
% 					 ymin=0,ymax=1] 
% 			\nextgroupplot[title={PTCH1, without masking},ylabel={FSC},xlabel={(a)}] 	
% 			 \addplot[black,very thick] table[x=x, y=y, col sep=comma]{figures/7795_unif/FSC_true.dat};	
% 			 \addplot[red,very thick,dashdotted] table[x=x, y=y, col sep=comma]{figures/7795_unif/FSC_joint.dat};
% 			 \addplot[blue,very thick,dashed] table[x=x, y=y, col sep=comma]{figures/7795_unif/FSC_approx.dat};
% 			 \addplot[darkgreen,very thick,dotted] table[x=x, y=y, col sep=comma]{figures/7795_unif/FSC_relion.dat};	
% 			 \addplot[magenta] table[x=x, y=y, col sep=comma]{figures/7795_unif/FSC_init.dat};	
% 		\nextgroupplot[yticklabels={,,},title={HJC, without masking},xlabel={(b)}] 	
% 			 \addplot[black,very thick] table[x=x, y=y, col sep=comma]{figures/3400_unif/FSC_true.dat};	
% 			 \addplot[red,very thick,dashdotted] table[x=x, y=y, col sep=comma]{figures/3400_unif/FSC_joint.dat};
% 			 \addplot[blue,very thick,dashed] table[x=x, y=y, col sep=comma] {figures/3400_unif/FSC_approx.dat};
% 			 \addplot[darkgreen,very thick,dotted] table[x=x, y=y, col sep=comma] {figures/3400_unif/FSC_relion.dat};	
% 			 \addplot[magenta] table[x=x, y=y, col sep=comma] {figures/3400_unif/FSC_init.dat};	
% 			 \legend{{\footnotesize True orient.},{\footnotesize Joint Recons.},{\footnotesize Unref. orient.},{\footnotesize Relion},{\footnotesize Init. Vol.}};
% 		\nextgroupplot[title={PTCH1, with masking},ylabel={FSC},xlabel={(c)}] 	
% 			 \addplot[black,very thick] table[x=x, y=y, col sep=comma]{figures/7795_unif/FSC_true_masked.dat};	
% 			 \addplot[red,very thick,dashdotted] table[x=x, y=y, col sep=comma]{figures/7795_unif/FSC_joint_masked.dat};
% 			 \addplot[blue,very thick,dashed] table[x=x, y=y, col sep=comma]{figures/7795_unif/FSC_approx.dat};
% 			 \addplot[darkgreen,very thick,dotted] table[x=x, y=y, col sep=comma]{figures/7795_unif/FSC_relion_masked.dat};	
% 			 \addplot[magenta] table[x=x, y=y, col sep=comma]{figures/7795_unif/FSC_init.dat};
% 		\nextgroupplot[yticklabels={,,},title={HJC with masking},xlabel={(d)}] 	
% 			 \addplot[black,very thick] table[x=x, y=y, col sep=comma]{figures/3400_unif/FSC_true_masked.dat};	
% 			 \addplot[red,very thick,dashdotted] table[x=x, y=y, col sep=comma]{figures/3400_unif/FSC_joint_masked.dat};
% 			 \addplot[blue,very thick,dashed] table[x=x, y=y, col sep=comma] {figures/3400_unif/FSC_approx.dat};
% 			 \addplot[darkgreen,very thick,dotted] table[x=x, y=y, col sep=comma] {figures/3400_unif/FSC_relion_masked.dat};	
% 			 \addplot[magenta] table[x=x, y=y, col sep=comma] {figures/3400_unif/FSC_init.dat};	
% 			 \legend{{\footnotesize True orient.},{\footnotesize Joint Recons.},{\footnotesize Unref. orient.},{\footnotesize Relion},{\footnotesize Init. Vol.}};
% 		\end{groupplot}
% 	\end{tikzpicture}
% 	\caption{Comparison between the FSC of the density maps obtained from several baselines and the ground-truth density map with masking (c)-(d) and without masking (a)-(b). The experimental setups  are identical to the ones used in Figure \ref{fig:fullmodel}.}
%     \label{fig:FSC_fullmodels}
% \end{figure*}
%-------------------------------------------------------

%FSC----------------------------------------------------
\begin{figure*}
\centering
	\begin{tikzpicture}
		\begin{groupplot}[group style={group size= 2 by 1, horizontal sep=0.8cm, vertical sep=2cm},     
	            	 legend pos= north east,        % Position de la légende dans les figures
					 legend style={at={(1.1,0.97)},legend cell align=left},
					 grid=both,                         % grid
    				 height=6cm,width=9cm,
					 ymin=-0.1,ymax=1,xmin=0] 
		\nextgroupplot[xmin=0,xmax=0.28,xtick={0,0.05,0.1,0.15,0.2,0.25},xticklabels={0,0.05,0.1,0.15,0.2,0.25},title={PTCH1},ylabel={FSC},xlabel={Spatial frequency ($1/\AA$)},xtick distance=0.05] 	
			 \addplot[black,very thick] table[x=x, y=y, col sep=comma]{new_results/fig56_with_relion/fsc_true_7795.dat};	
			 \addplot[red,very thick,dashdotted] table[x=x, y=y, col sep=comma]{new_results/fig56_with_relion/fsc_ours_7795.dat};
			 \addplot[blue,very thick,dashed] table[x=x, y=y, col sep=comma]{new_results/fig56_with_relion/fsc_approx_7795.dat};
			 \addplot[darkgreen,very thick,dotted] table[x=x, y=y, col sep=comma]{new_results/fig56_with_relion/fsc_relion_nopost_7795.dat};
			 \addplot[darkgreen,very thick] table[x=x, y=y, col sep=comma]{new_results/fig56_with_relion/fsc_relion_wpost_7795.dat};
			 \addplot[magenta] table[x=x, y=y, col sep=comma]{new_results/fig56_with_relion/fsc_init_7795.dat};
		\nextgroupplot[xmin=0,xmax=0.18,xtick={0,0.05,0.1,0.15},xticklabels={0,0.05,0.1,0.15},yticklabels={,,},title={HJC},xlabel={Spatial frequency ($1/\AA$)},xtick distance=0.05] 	
			 \addplot[black,very thick] table[x=x, y=y, col sep=comma]{new_results/fig56_with_relion/fsc_true.dat};
			 \addplot[red,very thick,dashdotted] table[x=x, y=y, col sep=comma]{new_results/fig56_with_relion/fsc_ours.dat};
			 \addplot[blue,very thick,dashed] table[x=x, y=y, col sep=comma] {new_results/fig56_with_relion/fsc_approx.dat};
			 \addplot[darkgreen,very thick,dotted] table[x=x, y=y, col sep=comma] {new_results/fig56_with_relion/fsc_relion_nopost.dat};
			 \addplot[darkgreen,very thick] table[x=x, y=y, col sep=comma] {new_results/fig56_with_relion/fsc_relion_wpost.dat};
			 \addplot[magenta] table[x=x, y=y, col sep=comma] {new_results/fig56_with_relion/fsc_init.dat};	
			 \legend{{\footnotesize True orient.},{\footnotesize Joint Recons.},{\footnotesize Unref. orient.},{\footnotesize Relion-wo-postpr.},{\footnotesize Relion-w-postpr.},{\footnotesize Init. Vol.}};
		\end{groupplot}
	\end{tikzpicture}
	\caption{Comparison between the FSC of the density maps obtained from several baselines and the ground-truth density map. \textcolor{black}{Relion-w-postpr (greed solid curve) and Relion-wo-postpr (green dashed curve) refer to the Relion results with and without post-processing, respectively. Note that Relion-wo-postpr is obtained after averaging the two half-maps.} The experimental setups  are identical to the ones used in Figure \ref{fig:fullmodel}.}
    \label{fig:FSC_fullmodels}
\end{figure*}

%CDF-angles------------------------------------------------------------------
% \begin{figure}%\centering
% \centering
% 	\begin{tikzpicture}
% 		\begin{groupplot}[group style={group size= 1 by 3,                      % taille du group plot
%     					  horizontal sep=0.5cm, vertical sep=0.5cm},     
% 	            	 legend pos= south east,        % Position de la légende dans les figures
% 					 legend style={legend cell align=left},
% 					 grid=both,                         % grid
%     				 height=4cm,width=8.8cm,
%     				 xmin=-40,xmax=40,
% 					 ymin=0,ymax=1] 
% 		\nextgroupplot[ylabel={CDF},xticklabels={,,}] 
% 		    \addplot[darkblue,very thick,dashed] table[x=x, y=y, col sep=comma]{new_results/fig56_with_relion/init_rot_3400_cdf.dat};
% 			 %\addplot[darkblue,very thick,dashed] table[x=x, y=y, col sep=comma]{figures/3400_unif/CDF_init1.dat};
% 			 \addplot[darkred,very thick] table[x=x, y=y, col sep=comma]{new_results/fig56_with_relion/ours_rot_3400_cdf.dat};
% 			 %\addplot[darkred,very thick] table[x=x, y=y, col sep=comma]{figures/3400_unif/CDF1.dat};
% 			 \addplot[darkgreen,very thick] table[x=x, y=y, col sep=comma]{new_results/fig56_with_relion/relion_rot_3400_cdf.dat};
% 			  \legend{{\footnotesize Initial $\theta_1$ },{\footnotesize Ours $\theta_1$ },{\footnotesize Relion $\theta_1$ }};
% 		\nextgroupplot[ylabel={CDF},xticklabels={,,}] 	
% 			 \addplot[darkblue,very thick,dashed] table[x=x, y=y, col sep=comma]{new_results/fig56_with_relion/init_tilt_3400_cdf.dat};
% 			 %\addplot[darkblue,very thick,dashed] table[x=x, y=y, col sep=comma]{figures/3400_unif/CDF_init2.dat};
% 			 %\addplot[darkred,very thick] table[x=x, y=y, col
% 			 %sep=comma]{figures/3400_unif/CDF2.dat};
% 			 \addplot[darkred,very thick] table[x=x, y=y, col sep=comma]{new_results/fig56_with_relion/ours_tilt_3400_cdf.dat};
% 			 \addplot[darkgreen,very thick] table[x=x, y=y, col sep=comma]{new_results/fig56_with_relion/relion_tilt_3400_cdf.dat};
% 			  \legend{{\footnotesize Initial $\theta_2$ },{\footnotesize Ours $\theta_2$ },{\footnotesize Relion $\theta_2$ }};
% 		\nextgroupplot[ylabel={CDF},xlabel={Error (degree)}] 
% 		     \addplot[darkblue,very thick,dashed] table[x=x, y=y, col sep=comma]{new_results/fig56_with_relion/init_psi_3400_cdf.dat};
% 			 %\addplot[darkblue,very thick,dashed] table[x=x, y=y, col sep=comma]{figures/3400_unif/CDF_init3.dat};
% 			 \addplot[darkred,very thick] table[x=x, y=y, col sep=comma]{new_results/fig56_with_relion/ours_psi_3400_cdf.dat};
% 			 %\addplot[darkred,very thick] table[x=x, y=y, col sep=comma]{figures/3400_unif/CDF3.dat};	
% 			 \addplot[darkgreen,very thick] table[x=x, y=y, col sep=comma]{new_results/fig56_with_relion/relion_psi_3400_cdf.dat};
% 			 \legend{{\footnotesize Initial $\theta_3$ },{\footnotesize Ours $\theta_3$ },{\footnotesize Relion $\theta_3$ }};
% 		\end{groupplot}
% 	\end{tikzpicture}
% \caption{Cumulative density function (CDF) of the differences between the true and refined projection orientations $\{\theta_{i,p}^{\mathrm{true}}-\theta_{i,p}^{\mathrm{rec}}\}_{p=1}^P$ (solid  curves) as well as the true and the initial projection orientations $\{\theta_{i,p}^{\mathrm{true}}-\theta_{i,p}^{\mathrm{init}}\}_{p=1}^P$ (dashed  curves). The experimental setup is identical to Figure \ref{fig:fullmodel} (HJC). \textcolor{blue}{Mona: change the caption accordingly.}}
% \label{fig:angle_refined}
% \end{figure}




%----------------------------------------------------------------------------
% \begin{figure}
% \centering
% \begin{tikzpicture}
% 	\pgfplotstableread[col sep=comma]{figures/3400_unif/Boxplot_unif.dat}\data
% 	% Boxplot groups columns, but we want rows
% 	%\pgfplotstabletranspose\datatransposed{\csvdata} 
% 	\begin{axis}[
% 		boxplot/draw direction = y,
% 		x axis line style = {opacity=0},
% 		axis x line* = bottom,
% 		axis y line = left,
% 		%enlarge y limits,
% 		%ymajorgrids,
% 		xtick = {1, 2, 3, 4},
% 		xtick style = {draw=none}, % Hide tick line
% 		xticklabel style = {align=center, font=\footnotesize, rotate=45,yshift=20pt,xshift=20pt},
% 		xticklabels = { $\{\mathbf{t}_{1,p}^\mathrm{true} - \mathbf{t}_{1,p}^\mathrm{init}\}_{p=1}^P$, $\{\mathbf{t}_{1,p}^\mathrm{true} - \mathbf{t}_{1,p}^\mathrm{rec}\}_{p=1}^P$, $\{\mathbf{t}_{2,p}^\mathrm{true} - \mathbf{t}_{2,p}^\mathrm{init}\}_{p=1}^P$, $\{\mathbf{t}_{2,p}^\mathrm{true} - \mathbf{t}_{2,p}^\mathrm{rec}\}_{p=1}^P$},
% 		ylabel = {},
% 		ytick = {-5,0,5},ymin=-5,ymax=5
% 	]
% 			\addplot+[boxplot, fill,darkblue , draw=black] table[y index=1] {\data};
% 			\addplot+[boxplot, fill,darkred,  draw=black, mark = x, mark options = {mark color=grey}] table[y index=0] {\data};
% 			\addplot+[boxplot, fill, darkblue, draw=black] table[y index=3] {\data};
% 			\addplot+[boxplot, fill,darkred,  draw=black, mark = x, mark options = {mark color=grey}] table[y index=2] {\data};
% 	\end{axis}
% \end{tikzpicture}
% \caption{The boxplot visualization of the differences between the true, refined, and initial shifts. The experimental setup is identical to Figure \ref{fig:fullmodel} (HJC). 
% }
% \label{fig:shift_refined}
% \end{figure}

\subsection{Visual Comparison}

We compare in Figure \ref{fig:fullmodel} the refined maps obtained using our join optimization scheme (Figure \ref{fig:fullmodel}-(d)) and the other methods (Figure \ref{fig:fullmodel}-(c,e,f)). In that experiment, the latent variables are initialized following the \textit{Init-1} model. 

As expected, the reconstruction fails when the unrefined 3D orientations are used (Figure~\ref{fig:fullmodel}-(c)). This confirms that angular refinement is required to achieve a successful reconstruction. Predictable as well is the fact that a perfect knowledge of the true 3D poses leads to a successful reconstruction (Figure~\ref{fig:fullmodel}-(e)).
It can be clearly seen that the results of our method (Figure \ref{fig:fullmodel}-(d)) closely resemble the reconstructed map resulting from perfect knowledge of the latent variables. This shows the ability of our method to appropriately refine the density map and the latent variables.

Figure~\ref{fig:fullmodel}-(f) contains the 3D density map refined by Relion. 
%The map contains high-frequency details that do not appear in the ground-truth density map. Moreover, 
We observe that the map refined through our method is more similar to the ground-truth density map than the Relion output.

\subsection{FSC Curves}

The FSC curves of the reconstructed maps are sketched in Figure~\ref{fig:FSC_fullmodels}. These curves confirm that our joint-optimization approach (red dash-dotted curve) is able to appropriately refine the low-resolution initial map. Its performance indeed closely approaches that of the reconstruction with perfect knowledge of 3D orientations (solid curve). Moreover, our framework outperforms the Relion outcome with and without post-processing (green curves).

% In addition, we can clearly see that masking the background noise improves the FSC. However, for our method, this improvement is marginal. This shows that the proposed method can be used without post-processing.




% the pdf plots
\begin{figure}%\centering
\centering
	\begin{tikzpicture}
		\begin{groupplot}[group style={group size= 1 by 3,                      % taille du group plot
    				horizontal sep=0.8cm, vertical sep=0.35cm},     
	            	 legend pos= north east,        % Position de la légende dans les figures
					 legend style={legend cell align=left},
					 grid=both,                         % grid
    				 height=4.8cm,width=8cm,
    				 xmin=-20,xmax=20,
					 ymin=0,ymax=0.6] 
		\nextgroupplot[ylabel={PDF},xticklabels={,,}] 	
			 \addplot[darkblue,very thick] table[x=x, y=y, col sep=comma]{new_results/fig56_with_relion/init_rot_3400.dat};	
			 \addplot[darkred,very thick] table[x=x, y=y, col sep=comma]{new_results/fig56_with_relion/ours_rot_3400.dat};
			 \addplot[darkgreen,very thick] table[x=x, y=y, col sep=comma]{new_results/fig56_with_relion/relion_rot_3400.dat};
			 \legend{{\footnotesize Initial $\theta_1$ },{\footnotesize Ours $\theta_1$ },{\footnotesize Relion $\theta_1$ }};
		\nextgroupplot[xticklabels={,,},ylabel={PDF}] 	
			 \addplot[darkblue,very thick] table[x=x, y=y, col sep=comma]{new_results/fig56_with_relion/init_tilt_3400.dat};	
			 \addplot[darkred,very thick] table[x=x, y=y, col sep=comma]{new_results/fig56_with_relion/ours_tilt_3400.dat};
			 \addplot[darkgreen,very thick] table[x=x, y=y, col sep=comma]{new_results/fig56_with_relion/relion_tilt_3400.dat};
			 %\legend{{\footnotesize Initial $\theta_2$ },{\footnotesize Ours $\theta_2$ },{\footnotesize Relion $\theta_2$ }};
		\nextgroupplot[xlabel={Error (degree)},ylabel={PDF}] 	
			 \addplot[darkblue,very thick] table[x=x, y=y, col sep=comma]{new_results/fig56_with_relion/init_psi_3400.dat};	
			 \addplot[darkred,very thick] table[x=x, y=y, col sep=comma]{new_results/fig56_with_relion/ours_psi_3400.dat};
			 \addplot[darkgreen,very thick] table[x=x, y=y, col sep=comma]{new_results/fig56_with_relion/relion_psi_3400.dat};
			 %\legend{{\footnotesize Initial $\theta_3$ },{\footnotesize Ours $\theta_3$ },{\footnotesize Relion $\theta_3$ }};
		\end{groupplot}
	\end{tikzpicture}
\caption{\color{black}Probability density function (PDF) of the differences between the true and refined projection orientations by our method $\{\theta_{i,p}^{\mathrm{true}}-\theta_{i,p}^{\mathrm{rec}}\}_{p=1}^P$ (red  curves), the true and refined projection orientations by Relion $\{\theta_{i,p}^{\mathrm{true}}-\theta_{i,p}^{\mathrm{Relion}}\}_{p=1}^P$ (green curves), as well as the true and the initial projection orientations $\{\theta_{i,p}^{\mathrm{true}}-\theta_{i,p}^{\mathrm{init}}\}_{p=1}^P$ (blue curves). The experimental setup is identical to Figure \ref{fig:fullmodel} (HJC). The x-axis is truncated between -20 and 20 degrees for the sake of clarity.}
\label{fig:angle_refined_hjc}
\end{figure}

% refined shifts
\begin{figure}%\centering
    \centering
	\begin{tikzpicture}
		\begin{groupplot}[group style={group size= 1 by 2,                      % taille du group plot
    				horizontal sep=0.5cm, vertical sep=0.35cm},     
	            	 legend pos= north east,        % Position de la légende dans les figures
					 legend style={legend cell align=left},
					 grid=both,                         % grid
    				 height=4.8cm,width=8cm,
    				 xmin=-10,xmax=10,
					 ymin=0,ymax=1] 
		\nextgroupplot[ylabel={PDF},xticklabels={,,}] 	
			 \addplot[darkblue,very thick] table[x=x, y=y, col sep=comma]{new_results/fig56_with_relion/init_shiftx_3400.dat};	
			 \addplot[darkred,very thick] table[x=x, y=y, col sep=comma]{new_results/fig56_with_relion/ours_shiftx_3400.dat};
			 \addplot[darkgreen,very thick] table[x=x, y=y, col sep=comma]{new_results/fig56_with_relion/relion_shiftx_3400.dat};
			 \legend{{\footnotesize Initial $t_1$ },{\footnotesize Ours $t_1$ },{\footnotesize Relion $t_1$ }};
		\nextgroupplot[ylabel={PDF},xlabel={Error (pixels)}] 	
			 \addplot[darkblue,very thick] table[x=x, y=y, col sep=comma]{new_results/fig56_with_relion/init_shifty_3400.dat};	
			 \addplot[darkred,very thick] table[x=x, y=y, col sep=comma]{new_results/fig56_with_relion/ours_shifty_3400.dat};
			 \addplot[darkgreen,very thick] table[x=x, y=y, col sep=comma]{new_results/fig56_with_relion/relion_shifty_3400.dat};
			 %\legend{{\footnotesize Initial $t_2$ },{\footnotesize Ours $t_2$ },{\footnotesize Relion $t_2$ }};
		\end{groupplot}
	\end{tikzpicture}
    \caption{\color{black} Probability density function (PDF) of the differences between the true and refined in-plane translations by our method $\{\mathbf{t}_{1,p}^\mathrm{true} - \mathbf{t}_{1,p}^\mathrm{rec}\}_{p=1}^P$ (red  curves), the true and refined in-plane translations by Relion $\{\mathbf{t}_{1,p}^\mathrm{true} - \mathbf{t}_{1,p}^\mathrm{Relion}\}_{p=1}^P$ (green curves), as well as the true and the initial in-plane translations $\{\mathbf{t}_{1,p}^\mathrm{true} - \mathbf{t}_{1,p}^\mathrm{init}\}_{p=1}^P$ (blue curves). The experimental setup is identical to Figure \ref{fig:fullmodel} (HJC).}
    \label{fig:shifts_refined_hjc}
\end{figure}

\subsection{Quality of Angular Refinement}
In Figure \ref{fig:angle_refined_hjc}, one finds the probability density function (PDF) of the differences between 1) the true and initial projection orientations (blue curve), 2) the true and refined projection orientations by our method (red curve), and 3) the true and refined projection orientations by Relion (green curve). The optimal PDF is obtained when all the differences are zero, up to a global rotation. The corresponding curve resembles a \textcolor{black}{delta} function that is one at zero, and zero elsewhere. Based on this, we observe that our proposed method performs well in recovering the projection orientations \textcolor{black}{and outperforms Relion}.

\textcolor{black}{Figure \ref{fig:shifts_refined_hjc} compares the PDF of the difference between 1) the true and initial in-plane translations (blue curve), 2) the true and refined in-plane translations by our method (red curve), and 3) the true and refined in-plane translations by Relion (green curve). Here as well, the figure demonstrates the ability of our method to refine in-plane translations, and its increased performance compared to Relion.}


% The comparison between the true and the recovered shifts is plotted in Figure \ref{fig:shift_refined_2}. The initial value for the in-plane translation is zero for all projection images. After refinement, the in-plane translations have converged to their true values for most projections as shown by the fact that the boxplot of errors is concentrated around zero. For a few projection images, though, the refined shift values is off. This is likely due to the non-convexity of the problem. 

\subsection{Convergence Results}

The evolution of the density map during refinement  is presented in Figure \ref{fig:alg_evolution}. The convergence in terms of resolution of our framework and  of two other baselines are shown in Figure~\ref{fig:fsc_evol}, where $r_c$ marks the radial frequency at which the FSC between the true and the reconstructed density map equals~$0.5$.

When the 3D projection orientations are perfectly known (solid curve), the reconstruction process achieves a high-resolution map in {\color{black} twenty} iterations. A key result is that our framework (dash-dotted curve) is able to converge to an almost equally-high resolution map starting from less-than-ideal 3D projection orientations. Once again, we observe failure when reconstructing with the unrefined set of projection orientations. This further confirms that refinement of the latent variables is vital to achieve a high-quality reconstruction of the map.  

\begin{figure}
    \centering
    \includegraphics[width = 1 \linewidth]{results/method_evol2.png}
    \caption{Evolution through iterations for the refinement of PTCH1. The experimental setup is the same as in  Figure \ref{fig:fullmodel}.}
    \label{fig:alg_evolution}
\end{figure}



\begin{figure}
    \centering
    		\begin{tikzpicture}
		\begin{axis}[legend pos= south east,        % Position de la légende dans les figures
					 legend style={legend cell align=left},
					 grid=both,                         % grid
				     set layers,cell picture=true,
					 ytick={0,0.1},
    				 height=6cm,width=8.8cm,
    				 xmin=0,xmax=40,
					 ymin=0,ymax=0.12,ylabel={$r_c$ ($1/\AA$)},xlabel=Iterations] 
					 \addplot[black,very thick] table[x=x, y=y, col sep=comma]{figures/3400_unif/evol_true_pixel.dat};	
					 \addplot[red,very thick,dashdotted] table[x=x, y=y, col sep=comma]{figures/3400_unif/evol_joint_pixel.dat};
					 \addplot[blue,very thick,dashed] table[x=x, y=y, col sep=comma]{figures/3400_unif/evol_approx_pixel.dat};	
			\legend{{True orient.},{Joint recons.},{Unref. orient.}};
		\end{axis}
	\end{tikzpicture}
    \caption{Evolution of $r_c$, the radial frequency at which the FSC equals $0.5$. Dash-dotted curve:  Our joint-reconstruction framework.  Solid curve: Reconstruction with true orientation projections. Dashed  curve: Reconstruction with unrefined orientation projections. The experimental setup is identical to Figure \ref{fig:fullmodel} (HJC). }
    \label{fig:fsc_evol}
\end{figure}

\begin{figure*}
    \centering
    \includegraphics[width=1 \linewidth]{figures/3400_2e4/3400_viz_2e4.png}
    \caption{\color{black} Reconstructions of HJC. {Left}: Samples of the noisy projection images.  Top row: 3D structures. Bottom row: Intensity maps of the central slice of the structures. The presented volumes are (a) the ground truth, (b) the initial map, (c) the output of our joint refinement approach after post-processing, (d) the output of Relion after post-processing. For this experiments, the latent variables are initialized following the \textit{Init-2} model using the results from Relion 3D ab-initio modeling. The parameters of this experiment are: $P=20000$, $\mathrm{SNR}_{\mathrm{data}} = -14.2 \, \textrm{dB}$, $m_{\textbf{t}} = 3$.
    }
    \label{fig:3400_viz_1e4}
\end{figure*}

% \begin{figure*}
%     \centering
%     \includegraphics[width=1 \linewidth]{figures/3400_1e4/3400_viz_1e4_reg.png}
%     \caption{\color{red} Reconstructions of HJC. {Left}: Samples of the noisy projection images.  Top row: 3D structures. Bottom row: Intensity maps of the central slice of the structures. The presented volumes are (a) the ground truth, (b) the initial map, (c) the output of our joint refinement approach after post-processing, (d) the output of Relion after post-processing. For this experiments, the latent variables are initialized following the \textit{Init-2} model using the results from Relion 3D ab-initio modeling. The parameters of this experiment are: $P=20000$, $\mathrm{SNR}_{\mathrm{data}} = -14.2 \, \textrm{dB}$, $m_{\textbf{t}} = 3$. \mz{for the experiment with 1e4 proj images+regularization.}
%     }
%     \label{fig:3400_viz_1e4_reg}
% \end{figure*}

% FSC curves
    \begin{figure}%\centering
    \centering
	\begin{tikzpicture}
		\begin{groupplot}[group style={group size= 1 by 1,                      % taille du group plot
    				horizontal sep=0.5cm, vertical sep=0.5cm},     
	            	 legend pos= north east,        % Position de la légende dans les figures
					 legend style={at={(1.03,1.02)},legend cell align=left},
					 grid=both,                         % grid
    				 height=7cm,width=9cm,
    				 xticklabels={-1,0,0.05,0.1,0.15,0.2,0.25},
    				 xmin=0,xmax=0.25,
					 ymin=-.1,ymax=1] 
		\nextgroupplot[xlabel={Spatial Frequency ($1/\AA$)},ylabel={FSC}] 	
			 \addplot[darkblue,very thick] table[x=x, y=y, col sep=comma]{figures/3400_2e4/fsc_init.dat};	
			 \addplot[darkred,very thick,dashed] table[x=x, y=y, col sep=comma]{figures/3400_2e4/fsc_ours_nopost.dat};
			 \addplot[darkred,very thick] table[x=x, y=y, col sep=comma]{figures/3400_2e4/fsc_ours_wpost.dat};
			 \addplot[darkgreen,very thick,dashed] table[x=x, y=y, col sep=comma]{figures/3400_2e4/fsc_relion_nopost.dat};
			 \addplot[darkgreen,very thick] table[x=x, y=y, col sep=comma]{figures/3400_2e4/fsc_relion_wpost.dat};
			 \legend{{\footnotesize Init. Vol. },{\footnotesize Joint Recons. wo. postpr},{\footnotesize Joint Recons. w. postpr},{\footnotesize Relion wo. postpr },{\footnotesize Relion w. postpr }};
		\end{groupplot}
	\end{tikzpicture}
    \caption{Comparison between the FSC of the density maps obtained from several baselines and the ground-truth density map. \textcolor{black}{Relion-w-postpr (green solid curve) and Relion-wo-postpr (green dashed curve) refer to the Relion results with and without post-processing, respectively. Note that, Relion-wo-postpr is obtained after averaging the two half-maps.} The experimental setups  are identical to the ones used in Figure \ref{fig:3400_viz_1e4}.}
    \label{fig:fsc_2e4}
    \end{figure}
    
%     \begin{figure}%\centering % with regularization
%     \centering
% 	\begin{tikzpicture}
% 		\begin{groupplot}[group style={group size= 1 by 1,                      % taille du group plot
%     				horizontal sep=0.5cm, vertical sep=0.5cm},     
% 	            	 legend pos= north east,        % Position de la légende dans les figures
% 					 legend style={at={(1.03,1.02)},legend cell align=left},
% 					 grid=both,                         % grid
%     				 height=7cm,width=9cm,
%     				 xticklabels={-1,0,0.05,0.1,0.15,0.2,0.25},
%     				 xmin=0,xmax=0.25,
% 					 ymin=-.1,ymax=1] 
% 		\nextgroupplot[xlabel={Spatial Frequency ($1/\AA$)},ylabel={FSC}] 	
% 			 \addplot[darkblue,very thick] table[x=x, y=y, col sep=comma]{figures/3400_2e4/fsc_init.dat};	
% 			 \addplot[darkred,very thick,dashed] table[x=x, y=y, col sep=comma]{figures/3400_1e4/fsc_ours_nopost_reg.dat};
% 			 \addplot[darkred,very thick] table[x=x, y=y, col sep=comma]{figures/3400_1e4/fsc_ours_wpost_reg.dat};
% 			 \addplot[darkgreen,very thick,dashed] table[x=x, y=y, col sep=comma]{figures/3400_1e4/fsc_relion_nopost_reg.dat};
% 			 \addplot[darkgreen,very thick] table[x=x, y=y, col sep=comma]{figures/3400_1e4/fsc_relion_wpost_reg.dat};
% 			 \legend{{\footnotesize Init. Vol. },{\footnotesize Joint Recons. wo. postpr},{\footnotesize Joint Recons. w. postpr},{\footnotesize Relion wo. postpr },{\footnotesize Relion w. postpr }};
% 		\end{groupplot}
% 	\end{tikzpicture}
%     \caption{Comparison between the FSC of the density maps obtained from several baselines and the ground-truth density map. \textcolor{red}{Relion-w-postpr (green solid curve) and Relion-wo-postpr (green dashed curve) refer to the Relion results with and without post-processing, respectively. Note that, Relion-wo-postpr is obtained after averaging the two half-maps.} The experimental setups  are identical to the ones used in Figure \ref{fig:3400_viz_1e4}. \mz{for the experiment with 1e4 proj images + regularization.}}
%     \label{fig:fsc_2e4}
%     \end{figure}

\subsection{Simulation of a Real Scenario}
\textcolor{black}{We then mimic a real scenario in which the output of the 3D \textit{ab initio} method provided by Relion  is used to initialize both the density map and the projection orientations. The in-plane translations are initialized with zeros. We use the same HJC structure to synthesize a volume with size $124\times124\times124$ and with a voxel size of $2 \AA$. The number of projection images is $20,000$ and the average SNR of the projection images is $-14.2 \textrm{dB}$. Examples of projection images are provided in Fig.~\ref{fig:3400_viz_1e4} (left most column).}

We  split the projection dataset in two halves and refine each half separately, starting from the same initial volume. Independent refinement of the two halves is a common approach in practice and has two main goals. First, by comparing the two refined half maps against one another, a convergence criterion is obtained. More precisely, we stop the refinement when the FSC between the two half maps fails to improve from one iteration to the next. Second, it reduces overfitting, especially in high-noise regimes. 

\textcolor{black}{A visual comparison of the density maps refined by our method and by Relion is presented in Fig.~\ref{fig:3400_viz_1e4} (c)-(e). Both results are post-processed by combining the half-maps and filtering out frequencies beyond the gold-standard FSC by applying a soft tight mask.}
% masked with the same soft tight mask to reduce the effect of background noise. For Relion, the half-maps are combined by filtering out frequencies beyond the gold-standard FSC. To post-process our refined half-maps Fig.~\ref{fig:3400_viz_1e4}-(d), we average them and apply a low-pass Gaussian filter with standard deviation of $2$. We found this post-processing approach to work better for our method than the post-processing options provided in Relion.
% \mz{Actually for the experiment with 20,000 projection images, I applied the same post-processing step to the final results of our method. This is also included in the FSC  and Fig. 9. Therefore, if you agree and think that the quality of the post-processed map from our method is good, we can keep it and mention that we apply the same post-processing to our method and Relion.}}

% \es{See my next comment}


\textcolor{black}{A quantitative comparison between our method and Relion based on FSC is provided in Fig.~\ref{fig:fsc_2e4}. Our method outperforms Relion both with and without post processing.}

\textcolor{black}{To assess the quality of the refined latent variables, we compute the PDF of the errors between the refined and the ground-truth projection orientations and in-plane translations. We do this for both our method and Relion, and display the comparisons in Fig.~\ref{fig:angle_refined_2e4} and~\ref{fig:shift_refined_2e4}. We observe that the proposed method enjoys comparable performance with Relion for the refinement of the projection orientations and in-plane translations.}

\textcolor{black}{Hence, while the proposed angular refinement offers a substantial gain over Relion in the proof-of-concept experiments, the difference here is less significant for a larger volume and a noisier regime. However, our framework could be further improved in several ways. An option would be to add regularization for the latent variable estimation. The proposed framework could also be combined with the multi-scale approach proposed in~\cite{donati2018fast} to perform angle refinements at coarser scales, which demonstrates increased robustness to noise. We expect that those extensions would further improve the performance of the method while keeping an attractive numerical complexity as demonstrated in Section~\ref{sec:ComplexityComparaison}. These extensions are to be addressed in future works.}

% , , 2) Relion has less outliers than our method for the refinement of the in-plane translations, which translates in a more peaked PDF in Fig.~\ref{fig:shift_refined_2e4}. We believe that the regularization term involved in the in-plane translation update steps helps improve the quality of the refined in-plane translations.} \mz{Added the last line, what do you think?}


% In addition, 
% The reconstruction results and the comparison with Relion are shown in Figure \ref{fig:real_scenario}, in which we also provide the FSC curve obtained when masking the outputs. In Figure \ref{fig:real_scenario}, \textit{Joint recons.} and \textit{Relion} correspond to the results of our joint reconstruction and Relion refinement with no post-processing other than averaging the two half-maps. Meanwhile,  \textit{Joint recons. (masked)} and \textit{Relion (masked)} are obtained after masking. The same mask is used for post-processing of both \textit{Joint recons.} and \textit{Relion}.


% \begin{itemize}
%     \item \textbf{Setting:} A density map generated from EMD-3400 using the method described in our paper but this time with higher resolution. Size of the volume = 124x124x124. Number of projection images = 10,000 (examples of projection images provided in Fig. 1). SNR = . No CTF. Examples of the projection images are provided in Fig.~\ref{fig:proj_3400}.
%     \item \textbf{Initialization:} We used the results of Relion ab-initio method to initialize both the density map and the projection angles. The in-plane translations are initialized with zeros.
%     \item \textbf{Our results and its comparison with Relion (quality of the density map):} The quality of the density map resulting from our refinement method is compared against the ground truth, the initial map and the results from Relion in Fig.~\ref{fig:3400_nonoise}. In addition, to quantify the performance of our method, we have presented Fig.~\ref{fig:fsc_3400_nonoise}, comparing the FSC between the ground truth density map and various density maps including initial map (blue curve), our refinement approach (red curve), and Relion (yellow curve).
    
%     \item \textbf{Our results and its comparison with Relion (quality of the refined latent variables):} Figure~\ref{fig:angles_refined_small_pdf} and~\ref{fig:in-plane-trans} compares the probability density function of the differences between the refined and initial projection angles and in-plane translations.

    % FSC curves
    % this is for the experiment with 1e4 projection images
%     \begin{figure}%\centering
%     \centering
% 	\begin{tikzpicture}
% 		\begin{groupplot}[group style={group size= 1 by 1,                      % taille du group plot
%     				horizontal sep=0.5cm, vertical sep=0.5cm},     
% 	            	 legend pos= north east,        % Position de la légende dans les figures
% 					 legend style={legend cell align=left},
% 					 grid=both,                         % grid
%     				 height=6cm,width=8cm,
%     				 xmin=0,xmax=0.25,
% 					 ymin=-.1,ymax=1] 
% 		\nextgroupplot[xlabel={Spatial Frequency},ylabel={FSC}] 	
% 			 \addplot[darkblue,very thick] table[x=x, y=y, col sep=comma]{figures/3400_1e4/fsc_init_hr.dat};	
% 			 \addplot[darkred,very thick] table[x=x, y=y, col sep=comma]{figures/3400_1e4/fsc_ours_hr.dat};
% 			 \addplot[darkgreen,very thick, dashed] table[x=x, y=y, col sep=comma]{figures/3400_1e4/fsc_relion_nopost_hr.dat};
% 			 \addplot[darkgreen,very thick] table[x=x, y=y, col sep=comma]{figures/3400_1e4/fsc_relion_wpost_hr.dat};
% 			 \legend{{\footnotesize Init. Vol. },{\footnotesize Joint Recons. },{\footnotesize Relion wo. postpr },{\footnotesize Relion w. postpr }};
% 		\end{groupplot}
% 	\end{tikzpicture}
%     \caption{Comparison between the FSC of the density maps obtained from several baselines and the ground-truth density map. \textcolor{red}{Relion-w-postpr (greed solid curve) and Relion-wo-postpr (green dashed curve) refer to the Relion results with and without post-processing respectively. Note that, Relion-wo-postpr is obtained after averaging the two half-maps.} The experimental setups  are identical to the ones used in Figure \ref{fig:3400_viz_1e4}.}
%     \label{fig:fsc_1e4}
%     \end{figure}
    


    % Refined angles results: experiment with 1e4 projection images
%     \begin{figure*}%\centering
%     \centering
% 	\begin{tikzpicture}
% 		\begin{groupplot}[group style={group size= 3 by 1,                      % taille du group plot
%     				horizontal sep=0.5cm, vertical sep=0.5cm},     
% 	            	 legend pos= north east,        % Position de la légende dans les figures
% 					 legend style={legend cell align=left},
% 					 grid=both,                         % grid
%     				 height=5cm,width=6.5cm,
%     				 xmin=-20,xmax=20,
% 					 ymin=0,ymax=0.25] 
% 		\nextgroupplot[xlabel={Error (degree)},ylabel={PDF}] 	
% 			 \addplot[darkblue,very thick] table[x=x, y=y, col sep=comma]{figures/3400_1e4/init_rot_hr.dat};	
% 			 \addplot[darkred,very thick] table[x=x, y=y, col sep=comma]{figures/3400_1e4/ours_rot_hr.dat};
% 			 \addplot[darkgreen,very thick] table[x=x, y=y, col sep=comma]{figures/3400_1e4/relion_rot_hr.dat};
% 			 \legend{{\footnotesize Initial $\theta_1$ },{\footnotesize Ours $\theta_1$ },{\footnotesize Relion $\theta_1$ }};
% 		\nextgroupplot[xlabel={Error (degree)},yticklabels={,,}] 	
% 			 \addplot[darkblue,very thick] table[x=x, y=y, col sep=comma]{figures/3400_1e4/init_tilt_hr.dat};	
% 			 \addplot[darkred,very thick] table[x=x, y=y, col sep=comma]{figures/3400_1e4/ours_tilt_hr.dat};
% 			 \addplot[darkgreen,very thick] table[x=x, y=y, col sep=comma]{figures/3400_1e4/relion_tilt_hr.dat};
% 			 \legend{{\footnotesize Initial $\theta_2$ },{\footnotesize Ours $\theta_2$ },{\footnotesize Relion $\theta_2$ }};
% 		\nextgroupplot[xlabel={Error (degree)},yticklabels={,,}] 	
% 			 \addplot[darkblue,very thick] table[x=x, y=y, col sep=comma]{figures/3400_1e4/init_psi_hr.dat};	
% 			 \addplot[darkred,very thick] table[x=x, y=y, col sep=comma]{figures/3400_1e4/ours_psi_hr.dat};
% 			 \addplot[darkgreen,very thick] table[x=x, y=y, col sep=comma]{figures/3400_1e4/relion_psi_hr.dat};
% 			 \legend{{\footnotesize Initial $\theta_3$ },{\footnotesize Ours $\theta_3$ },{\footnotesize Relion $\theta_3$ }};
% 		\end{groupplot}
% 	\end{tikzpicture}
%     \caption{Probability density function (PDF) of the differences between the true and refined projection orientations by our method $\{\theta_{i,p}^{\mathrm{true}}-\theta_{i,p}^{\mathrm{rec}}\}_{p=1}^P$ (red  curves), the true and refined projection orientations by Relion (green curves), as well as the true and the initial projection orientations $\{\theta_{i,p}^{\mathrm{true}}-\theta_{i,p}^{\mathrm{init}}\}_{p=1}^P$ (blue curves). The experimental setup is identical to Figure \ref{fig:3400_viz_1e4}.}
%     \label{fig:angle_refined}
%     \end{figure*}
    
%     % refined shifts
%     \begin{figure*}%\centering
%     \centering
% 	\begin{tikzpicture}
% 		\begin{groupplot}[group style={group size= 2 by 1,                      % taille du group plot
%     				horizontal sep=0.5cm, vertical sep=0.5cm},     
% 	            	 legend pos= north east,        % Position de la légende dans les figures
% 					 legend style={legend cell align=left},
% 					 grid=both,                         % grid
%     				 height=5cm,width=6.5cm,
%     				 xmin=-6,xmax=6,
% 					 ymin=0,ymax=0.2] 
% 		\nextgroupplot[xlabel={Error (\textcolor{green}{TODO})},ylabel={PDF}] 	
% 			 \addplot[darkblue,very thick] table[x=x, y=y, col sep=comma]{figures/3400_1e4/init_shiftx_hr.dat};	
% 			 \addplot[darkred,very thick] table[x=x, y=y, col sep=comma]{figures/3400_1e4/ours_shiftx_hr.dat};
% 			 \addplot[darkgreen,very thick] table[x=x, y=y, col sep=comma]{figures/3400_1e4/relion_shiftx_hr.dat};
% 			 \legend{{\footnotesize Initial $t_1$ },{\footnotesize Ours $t_1$ },{\footnotesize Relion $t_1$ }};
% 		\nextgroupplot[xlabel={Error (\textcolor{green}{TODO})},yticklabels={,,}] 	
% 			 \addplot[darkblue,very thick] table[x=x, y=y, col sep=comma]{figures/3400_1e4/init_shifty_hr.dat};	
% 			 \addplot[darkred,very thick] table[x=x, y=y, col sep=comma]{figures/3400_1e4/ours_shifty_hr.dat};
% 			 \addplot[darkgreen,very thick] table[x=x, y=y, col sep=comma]{figures/3400_1e4/relion_shifty_hr.dat};
% 			 \legend{{\footnotesize Initial $t_2$ },{\footnotesize Ours $t_2$ },{\footnotesize Relion $t_2$ }};
% 		\end{groupplot}
% 	\end{tikzpicture}
%     \caption{Probability density function (PDF) of the differences between the true and refined in-plane translations by our method $\{\mathbf{t}_{1,p}^\mathrm{true} - \mathbf{t}_{1,p}^\mathrm{rec}\}_{p=1}^P$ (red  curves), the true and refined in-plane translations by Relion $\{\mathbf{t}_{1,p}^\mathrm{true} - \mathbf{t}_{1,p}^\mathrm{Relion}\}_{p=1}^P$ (green curves), as well as the true and the initial in-plane translations $\{\mathbf{t}_{1,p}^\mathrm{true} - \mathbf{t}_{1,p}^\mathrm{init}\}_{p=1}^P$ (blue curves). The experimental setup is identical to Figure \ref{fig:3400_viz_1e4}.}
%     \label{fig:shift_refined}
%     \end{figure*}
    
    % refined angles, experiment with 2e4 projection images
    \begin{figure}%\centering
    \centering
	\begin{tikzpicture}
		\begin{groupplot}[group style={group size= 1 by 3,                      % taille du group plot
    				horizontal sep=0.5cm, vertical sep=0.35cm},     
	            	 legend pos= north east,        % Position de la légende dans les figures
					 legend style={legend cell align=left},
					 grid=both,                         % grid
    				 height=4.8cm,width=8cm,
    				 xmin=-20,xmax=20,
					 ymin=0,ymax=0.25] 
		\nextgroupplot[ylabel={PDF},xticklabels={,,}] 	
			 \addplot[darkblue,very thick] table[x=x, y=y, col sep=comma]{figures/3400_2e4/init_rot_2e4.dat};	
			 \addplot[darkred,very thick] table[x=x, y=y, col sep=comma]{figures/3400_2e4/ours_rot_2e4.dat};
			 \addplot[darkgreen,very thick] table[x=x, y=y, col sep=comma]{figures/3400_2e4/relion_rot.dat};
			 \legend{{\footnotesize Initial $\theta_1$ },{\footnotesize Ours $\theta_1$ },{\footnotesize Relion $\theta_1$ }};
		\nextgroupplot[ylabel={PDF},xticklabels={,,}] 	
			 \addplot[darkblue,very thick] table[x=x, y=y, col sep=comma]{figures/3400_2e4/init_tilt_2e4.dat};	
			 \addplot[darkred,very thick] table[x=x, y=y, col sep=comma]{figures/3400_2e4/ours_tilt_2e4.dat};
			 \addplot[darkgreen,very thick] table[x=x, y=y, col sep=comma]{figures/3400_2e4/relion_tilt.dat};
			 %\legend{{\footnotesize Initial $\theta_2$ },{\footnotesize Ours $\theta_2$ },{\footnotesize Relion $\theta_2$ }};
		\nextgroupplot[ylabel={PDF},xlabel={Error (degree)}] 	
			 \addplot[darkblue,very thick] table[x=x, y=y, col sep=comma]{figures/3400_2e4/init_psi_2e4.dat};	
			 \addplot[darkred,very thick] table[x=x, y=y, col sep=comma]{figures/3400_2e4/ours_psi_2e4.dat};
			 \addplot[darkgreen,very thick] table[x=x, y=y, col sep=comma]{figures/3400_2e4/relion_psi.dat};
			 %\legend{{\footnotesize Initial $\theta_3$ },{\footnotesize Ours $\theta_3$ },{\footnotesize Relion $\theta_3$ }};
		\end{groupplot}
	\end{tikzpicture}
    \caption{\textcolor{black}{Probability density function (PDF) of the differences between the true and refined projection orientations by our method $\{\theta_{i,p}^{\mathrm{true}}-\theta_{i,p}^{\mathrm{rec}}\}_{p=1}^P$ (red  curves), the true and refined projection orientations by Relion (green curves), as well as the true and the initial projection orientations $\{\theta_{i,p}^{\mathrm{true}}-\theta_{i,p}^{\mathrm{init}}\}_{p=1}^P$ (blue curves). The experimental setup is identical to Figure \ref{fig:3400_viz_1e4}.}}
    \label{fig:angle_refined_2e4}
    \end{figure}
    
%     % refined angles, experiment with 1e4 projection images + regularization
%     \begin{figure}%\centering
%     \centering
% 	\begin{tikzpicture}
% 		\begin{groupplot}[group style={group size= 1 by 3,                      % taille du group plot
%     				horizontal sep=0.5cm, vertical sep=0.35cm},     
% 	            	 legend pos= north east,        % Position de la légende dans les figures
% 					 legend style={legend cell align=left},
% 					 grid=both,                         % grid
%     				 height=4.8cm,width=8cm,
%     				 xmin=-20,xmax=20,
% 					 ymin=0,ymax=0.25] 
% 		\nextgroupplot[ylabel={PDF},xticklabels={,,}] 	
% 			 \addplot[darkblue,very thick] table[x=x, y=y, col sep=comma]{figures/3400_1e4/init_rot_1e4.dat};	
% 			 \addplot[darkred,very thick] table[x=x, y=y, col sep=comma]{figures/3400_1e4/ours_rot_1e4.dat};
% 			 \addplot[darkgreen,very thick] table[x=x, y=y, col sep=comma]{figures/3400_1e4/relion_rot_1e4.dat};
% 			 \legend{{\footnotesize Initial $\theta_1$ },{\footnotesize Ours $\theta_1$ },{\footnotesize Relion $\theta_1$ }};
% 		\nextgroupplot[ylabel={PDF},xticklabels={,,}] 	
% 			 \addplot[darkblue,very thick] table[x=x, y=y, col sep=comma]{figures/3400_1e4/init_tilt_1e4.dat};	
% 			 \addplot[darkred,very thick] table[x=x, y=y, col sep=comma]{figures/3400_1e4/ours_tilt_1e4.dat};
% 			 \addplot[darkgreen,very thick] table[x=x, y=y, col sep=comma]{figures/3400_1e4/relion_tilt_1e4.dat};
% 			 %\legend{{\footnotesize Initial $\theta_2$ },{\footnotesize Ours $\theta_2$ },{\footnotesize Relion $\theta_2$ }};
% 		\nextgroupplot[ylabel={PDF},xlabel={Error (degree)}] 	
% 			 \addplot[darkblue,very thick] table[x=x, y=y, col sep=comma]{figures/3400_1e4/init_psi_1e4.dat};	
% 			 \addplot[darkred,very thick] table[x=x, y=y, col sep=comma]{figures/3400_1e4/ours_psi_1e4.dat};
% 			 \addplot[darkgreen,very thick] table[x=x, y=y, col sep=comma]{figures/3400_1e4/relion_psi_1e4.dat};
% 			 %\legend{{\footnotesize Initial $\theta_3$ },{\footnotesize Ours $\theta_3$ },{\footnotesize Relion $\theta_3$ }};
% 		\end{groupplot}
% 	\end{tikzpicture}
%     \caption{Probability density function (PDF) of the differences between the true and refined projection orientations by our method $\{\theta_{i,p}^{\mathrm{true}}-\theta_{i,p}^{\mathrm{rec}}\}_{p=1}^P$ (red  curves), the true and refined projection orientations by Relion (green curves), as well as the true and the initial projection orientations $\{\theta_{i,p}^{\mathrm{true}}-\theta_{i,p}^{\mathrm{init}}\}_{p=1}^P$ (blue curves). The experimental setup is identical to Figure \ref{fig:3400_viz_1e4}. \mz{this is for the experiment with 1e4 projection images and regularization.}}
%     \label{fig:angle_refined_1e4}
%     \end{figure}
    
    % refined shifts for experiment with 2e4 projection images
    \begin{figure}%\centering
    \centering
	\begin{tikzpicture}
		\begin{groupplot}[group style={group size= 1 by 2,                      % taille du group plot
    				horizontal sep=0.5cm, vertical sep=0.35cm},     
	            	 legend pos= north east,        % Position de la légende dans les figures
					 legend style={legend cell align=left},
					 grid=both,                         % grid
    				 height=4.8cm,width=8cm,
    				 xmin=-6,xmax=6,
					 ymin=0,ymax=0.2] 
		\nextgroupplot[ylabel={PDF},yticklabels={-1,0,0.05,0.1,0.15,0.2},,xticklabels={,,}] 	
			 \addplot[darkblue,very thick] table[x=x, y=y, col sep=comma]{figures/3400_2e4/init_shiftx_2e4.dat};	
			 \addplot[darkred,very thick] table[x=x, y=y, col sep=comma]{figures/3400_2e4/ours_shiftx_2e4.dat};
			 %\addplot[darkred,very thick,dashed] table[x=x, y=y, col sep=comma]{figures/3400_1e4/ours_shiftx_reg.dat};
			 \addplot[darkgreen,very thick] table[x=x, y=y, col sep=comma]{figures/3400_2e4/relion_shiftx_2e4.dat};
			 \legend{{\footnotesize Initial $t_1$ },{\footnotesize Ours $t_1$ },{\footnotesize Relion $t_1$ }};
		\nextgroupplot[ylabel={PDF},xlabel={Error (pixels)},yticklabels={-1,0,0.05,0.1,0.15,0.2}] 	
			 \addplot[darkblue,very thick] table[x=x, y=y, col sep=comma]{figures/3400_2e4/init_shifty_2e4.dat};	
			 \addplot[darkred,very thick] table[x=x, y=y, col sep=comma]{figures/3400_2e4/ours_shifty_2e4.dat};
			 %\addplot[darkred,very thick,dashed] table[x=x, y=y, col sep=comma]{figures/3400_1e4/ours_shifty_reg.dat};
			 \addplot[darkgreen,very thick] table[x=x, y=y, col sep=comma]{figures/3400_2e4/relion_shifty_2e4.dat};
			\legend{{\footnotesize Initial $t_2$ },{\footnotesize Ours $t_2$ },{\footnotesize Relion $t_2$ }};
		\end{groupplot}
	\end{tikzpicture}
    \caption{\textcolor{black}{Probability density function (PDF) of the differences between the true and refined in-plane translations by our method $\{\mathbf{t}_{1,p}^\mathrm{true} - \mathbf{t}_{1,p}^\mathrm{rec}\}_{p=1}^P$ (red  curves), the true and refined in-plane translations by Relion $\{\mathbf{t}_{1,p}^\mathrm{true} - \mathbf{t}_{1,p}^\mathrm{Relion}\}_{p=1}^P$ (green curves), as well as the true and the initial in-plane translations $\{\mathbf{t}_{1,p}^\mathrm{true} - \mathbf{t}_{1,p}^\mathrm{init}\}_{p=1}^P$ (blue curves). The experimental setup is identical to Figure \ref{fig:3400_viz_1e4}.}}
    \label{fig:shift_refined_2e4}
    \end{figure}
    
%     % refined shifts for experiment with 1e4 projection images + added reguarization on the shifts
%     \begin{figure}%\centering
%     \centering
% 	\begin{tikzpicture}
% 		\begin{groupplot}[group style={group size=1 by 2,                      % taille du group plot
%     				horizontal sep=0.5cm, vertical sep=0.35cm},     
% 	            	 legend pos= north east,        % Position de la légende dans les figures
% 					 legend style={legend cell align=left},
% 					 grid=both,                         % grid
%     				 height=4.8cm,width=8cm,
%     				 xmin=-6,xmax=6,
% 					 ymin=0,ymax=0.2] 
% 		\nextgroupplot[ylabel={PDF},xticklabels={,,},yticklabels={-1,0,0.05,0.1,0.15,0.2}] 	
% 			 \addplot[darkblue,very thick] table[x=x, y=y, col sep=comma]{figures/3400_2e4/init_shiftx_2e4.dat};	
% 			 \addplot[darkred,very thick] table[x=x, y=y, col sep=comma]{figures/3400_1e4/ours_shiftx_reg.dat};
% 			 \addplot[darkgreen,very thick] table[x=x, y=y, col sep=comma]{figures/3400_1e4/relion_shiftx_1e4.dat};
% 			 \legend{{\footnotesize Initial $t_1$ },{\footnotesize Ours $t_1$ },{\footnotesize Relion $t_1$ }};
% 		\nextgroupplot[ylabel={PDF},xlabel={Error (pixels)},yticklabels={-1,0,0.05,0.1,0.15,0.2}] 	
% 			 \addplot[darkblue,very thick] table[x=x, y=y, col sep=comma]{figures/3400_2e4/init_shifty_2e4.dat};	
% 			 \addplot[darkred,very thick] table[x=x, y=y, col sep=comma]{figures/3400_1e4/ours_shifty_reg.dat};
% 			 \addplot[darkgreen,very thick] table[x=x, y=y, col sep=comma]{figures/3400_1e4/relion_shifty_1e4.dat};
% 			 %\legend{{\footnotesize Initial $t_2$ },{\footnotesize Ours $t_2$ },{\footnotesize Relion $t_2$ }};
% 		\end{groupplot}
% 	\end{tikzpicture}
%     \caption{Probability density function (PDF) of the differences between the true and refined in-plane translations by our method $\{\mathbf{t}_{1,p}^\mathrm{true} - \mathbf{t}_{1,p}^\mathrm{rec}\}_{p=1}^P$ (red  curves), the true and refined in-plane translations by Relion $\{\mathbf{t}_{1,p}^\mathrm{true} - \mathbf{t}_{1,p}^\mathrm{Relion}\}_{p=1}^P$ (green curves), as well as the true and the initial in-plane translations $\{\mathbf{t}_{1,p}^\mathrm{true} - \mathbf{t}_{1,p}^\mathrm{init}\}_{p=1}^P$ (blue curves). The experimental setup is identical to Figure \ref{fig:3400_viz_1e4}. \mz{The new results for our method are from the latest experiment I ran with 10,000 projection images with regularization added to the shifts. In this one we can see that we no longer have a lot of outliers as the one in Fig. 12. However, this experiment is with 10,000 projection images as the one with 20,000 proj images would have taken longer to finish. What do you think? Shall we keep this one instead of Fig.12 and then in the final version, we will update it with the results with 20,000 projection images.}}
%     \label{fig:shift_refined_2e4}
%     \end{figure}


% Our goal here is to mimic a real scenario in which we use the output of the 3D \textit{ab initio} method provided by Relion as initial map and where we initialize the orientations using the \textit{Init-2} model. 

% We  split the projection dataset in two halves and refine each half separately, starting from the same initial volume. Independent refinement of the two halves is a common approach in practice and has two main goals. First, by comparing the two refined half maps against one another, a convergence criterion is obtained. More precisely, we stop the refinement when the FSC between the two half maps fails to improve from one iteration to the next. Second, it reduces overfitting, especially in high-noise regimes. 

% The reconstruction results and the comparison with Relion are shown in Figure \ref{fig:real_scenario}, in which we also provide the FSC curve obtained when masking the outputs. In Figure \ref{fig:real_scenario}, \textit{Joint recons.} and \textit{Relion} correspond to the results of our joint reconstruction and Relion refinement with no post-processing other than averaging the two half-maps. Meanwhile,  \textit{Joint recons. (masked)} and \textit{Relion (masked)} are obtained after masking. The same mask is used for post-processing of both \textit{Joint recons.} and \textit{Relion}.

% We see that 1) both the visual comparisons and the FSC curves in Figure \ref{fig:real_scenario} confirm that our approach provides a better map compared to Relion when starting from the same initial map and with no post-processing (\textit{i.e.}, masking) applied on the final outputs, 2) performing post-processing improves the FSC, 3) after masking, our method and Relion have comparable performances in terms of FSC, 4) although performing similarly  in terms of FSC, the SNR of our refined density map outperforms Relion by a large margin. While the texture of our density map  is very close to the ground-truth, Relion produces a map that contains many objectionable  high-frequency components. This does not appear in the FSC comparison but is clearly captured by the SNR metric.

% \begin{figure}
%     \centering
%     \hspace{0.8cm}\includegraphics[width = 0.8 \linewidth]{results/real_scenario_snr.png}
%     \begin{tikzpicture}
% 		\begin{axis}[legend pos= north east,        % Position de la légende dans les figures
% 					 legend style={nodes={scale=0.75, transform shape}, legend cell align=left},
% 					 grid=both,                         % grid
% 				     set layers,cell picture=true,
% 					 %xtick={0.00001,0.001,0.1,10,1000},
%     				 height=6cm,width=8.8cm,
%     				 xmin=0,xmax=0.5,
% 					 ymin=0,ymax=1,ylabel={FSC}] 
% 					 \addplot[red,very thick,dashdotted] table{figures/FSC_Real_Joint.dat};
% 					 \addplot[red,very thick] table[x=x, y=y, col sep=comma]{figures/FSC_Real_Joint_masked.dat};
% 					 \addplot[darkgreen,very thick,dotted] table{figures/FSC_Real_Relion.dat};
% 					 \addplot[darkgreen,very thick] table[x=x, y=y, col sep=comma]{figures/FSC_Real_Relion_masked.dat};
% 				% 	 \addplot[darkblue,very thick,dotted] table{figures/masked_joint.dat};
% 			\legend{{Joint recons.},{Joint recons. (masked)},{Relion},{Relion (masked)}};
% 		\end{axis}
% 	\end{tikzpicture}
%     \caption{Refined density maps based on our method and Relion. Top and middle rows: Visual comparison.
%     Bottom row:  FSC plot of the two reconstructions, where the horizontal axis marks the radius of the spherical shell in the frequency domain. The average SNR of the projection images is $-10.57$ dB, and $P=1000$.
%     }
%     \label{fig:fsc_1e4}
% \end{figure}



==> CryoEM-Joint Reconstruction/sections/6-conclusion.tex <==
\label{sec:conclusion}

We propose a variational 3D refinement framework for single-particle cryo-electron microscopy that jointly refines the density map and the 3D  projection orientations. The refinement of the orientations on the continuum does away with the computationally expensive projection-matching steps. We take alternating steps to update the density map and the latent variables. Steps of the classical method known as the alternating-direction method of multipliers are used to update the density map, while the latent variables are updated through gradient-descent. Our results demonstrate the ability of our framework to refine an approximate map from inaccurate 3D projection orientations. In addition, we show that the resolution of the refined map using our method closely approaches that of the map reconstructed with perfect knowledge of the 3D orientations.

